From X to Pi; Representing the Classical Sequent Calculus in the Pi-calculus

We study the Pi-calculus, enriched with pairing and non-blocking input, and define a notion of type assignment that uses the type constructor "arrow". We encode the circuits of the calculus X into this variant of Pi, and show that all reduction (cut-elimination) and assignable types are preserved. Since X enjoys the Curry-Howard isomorphism for Gentzen's calculus LK, this implies that all proofs in LK have a representation in Pi.

==> PiXmacros.tex <==
%{([
\makeatletter

% \mathrel \mathbin \mathop \mathord

\def\SetCtr#1#2{\global#1#2\relax}
\def\Adv#1#2{\advance#1#2\relax}

\setlength {\unitlength} {1\point}

\def \AppBis{\mathrel{\stackrel{\sim}{=}}}
 \def \PiC {$\Red `p$-cal\-cu\-lus}

\omtrue

 \def \tab{\hspace*{7.5mm}}

\def \proc#1{\mbox{\itsf #1\skp}}

\ifmycolour \newrgbcolor{picolour}{0 0 .9}\else\newrgbcolor{picolour}{0 0 0}\fi
% \def \picolour{\picol}
 \def \piterm#1 {{\picolour #1}}
 \def \process #1 {{\picolour #1}}
 \def \procPa'{\proc{P'}}
 \def \procP {\@ifnextchar{'}{\procPa}{\proc{P}}}
 \def \procQa'{\proc{Q'}}
 \def \procQ {\@ifnextchar{'}{\procQa}{\proc{Q}}}
 \def \procRa'{\proc{R'}}
 \def \procR {\@ifnextchar{'}{\procRa}{\proc{R}}}
 \def \procAa'{\proc{A'}}
 \def \procA {\@ifnextchar{'}{\procAa}{\proc{A}}}


 \def \leftbr{\psset{unit=1\point,linewidth=.45\point}%{,linecolor=picolour}%
\psline{c-c}(0,2.5)(1.5,6)%
\psline{c-c}(0,2.5)(1.5,-1)%
\kern2.5\point
}
 \def \rightbr{\psset{unit=1\point,linewidth=0.45\point}%{,linecolor=picolour}%
\kern2.5\point
\psline{c-c}(0,2.5)(-1.5,6)%
\psline{c-c}(0,2.5)(-1.5,-1)%
}

 \def \PiPairbr<#1,#2> {\ifmycolour\psset{linecolor=picolour}\else
\psset{linecolor=black}\fi {\leftbr{#1}{,}{#2}\rightbr}}%
 \def \PiPairBr(#1,#2){\ifmycolour\psset{linecolor=picolour}\else
\psset{linecolor=black}\fi {\leftbr{#1}{,}{#2}\rightbr}}%
 \def \PiPair{\@ifnextchar({\PiPairBr}{\PiPairbr}}%


 \def \InPoint #1 (#2) . {\picolour #1 (\hspace*{-.5\point}#2\hspace*{-.5\point})\hspace*{.1pt}.\hspace*{1.5pt}}
 \def \InTwo #1 (#2) {\@ifnextchar{.}%
 	{\InPoint {#1} ({#2}) }
	{{\picolour {#1} (\hspace*{-.5\point}{#2}\hspace*{-.5\point})}}
}
 \def \InAuxPair #1 (#2,#3) { \InTwo #1 (#2{,}#3) }
 \def \InAux #1 (#2{\@ifnextchar,{\InAuxPair #1 (#2}{\InTwo #1 (#2}}%))
 \def \In #1 {\@ifnextchar({\InAux {#1} }{#1}}%)

 \def \Use#1{\picolour \langle \hspace*{-.25\point}{ #1 }\hspace*{-.25\point}\rangle }
 \def \baseOut #1<#2>{\PiOverline{#1}\Use{#2}}
 \def \OutPoint #1<#2>.{\baseOut{#1}<{#2}>\hspace*{.5pt}.\hspace*{1.5pt}}
 \def \OutTwo #1<#2>{\@ifnextchar{.}{\OutPoint {#1}<{#2}>}{\baseOut{#1}<{#2}>}}
 \def \NewOut #1<#2>{\baseOut{#1}<{#2}>}
 \def \OutAux #1{\@ifnextchar({\NewOut{#1}}{\PiOverline{#1}}}%)
 \def \OutTwoPair #1 <#2,#3> {\baseOut{#1}<{#2{,}#3}>}
 \def \OutBux #1 <#2{\@ifnextchar,{\OutTwoPair #1 <#2}{\baseOut {#1} <#2}}
 \def \Out #1 {\@ifnextchar<{ \OutBux {#1} }{ \OutAux {#1} }}
%
 \def \BangUn_#1{{!}_{#1} \hskp}
 \def \Bang {\picolour \@ifnextchar_{\BangUn}{{!} \skp}}
% \def \Bang #1{\setbox124=\hbox{$#1$}%
%{\picolour !}\ifdim\wd124>4em{{\picolour \,<{#1}>}}\else{{\picolour \,{#1}}}\fi}
 \def \RepBr <#1> {\picolour {!}\skipper <#1>}
 \def \RepNoBr #1 {\picolour {!}\skipper {#1}}
 \def \Rep{\@ifnextchar({\RepBr}{\RepNoBr}}

 \def \NewDL #1 {\picolour %\hspace*{-.5\point}
(\hspace*{-.5\point}\nu \hspace*{.5\point} {#1}\hspace*{-.5\point})\skp}
 \def \NewTwo #1 (#2){\NewDL #1 (#2)}
 \def \New #1 {\@ifnextchar({\NewTwo {#1} }{\NewDL {#1} }}%)
 \def \NewA #1 {\picolour (\hspace*{-.5\point}\nu \hspace*{.5\point} {#1}\hspace*{-.5\point})\skp}
%
 \def \Zero {\proc{0}} % {\textrm{\bf 0}}
 \def \Choice{\mathop{\picolour +}}
% \def \Par{\skp{\picolour{\mbox{\large$\mid$}}}\skp}
 \def \Par{\mathbin{\picolour{\mbox{\large$\mid$}}}}
 \def \Arg{\kern-1\point{w}\kern-1\point}
% \def \Eq#1=#2 {\In {#1} . \Out {#2} }
 \def \Eq#1=#2 {{#1}{\rm =}{#2}}
 \def \EqX#1=#2 {\In {#1} (w) . \Out {#2} <w> }
 \def \BEq#1=#2 {\Bang {#1}{\rm =}{#2}}

 \def \forwarder{\psset{unit=1\point,linewidth=0.35\point}%{,linecolor=Bluecol}
\hbox{\put(-1.5,2.5){%
\psline{c-c}(2.5,0)(5.3,0)%
\psline{c-c}(7,0)(5.3,1.2)%
\psline{c-c}(7,0)(5.3,-1.2)
\pscurve{c-c}(5.3,1.2)(5.5,0)(5.3,-1.2)
}}\kern7\point}
 \def \Eq#1=#2 {{\picolour {#1}\forwarder{#2}}}
 \def \BEq#1=#2 {\Bang \Eq{#1}={#2} }
 \def \EqX#1=#2 {\In {#1} (w) . \Out {#2} <w> }

 \def \Let{\@ifnextchar){\textsl{let}}{\Letaux }}
 \def \Letaux{\@ifnextchar<{\Letterm }{\textsl{let}}}
 \def \Letterm <#1,#2> = #3 in #4{{\picolour \textsl{let }\PiPair<#1,#2> = {#3}\textsl{ in }{#4}}}
 \def \AddLet #1 = #2 in #3 {\textsl{let }#1 = {#2}\textsl{ in }{#3}}

\newcount \StrW
\newcount \StrH
 \def \strikethrough#1{\setbox112=\hbox{$#1$}%
\psset{unit=\unitlength}
\StrW\wd112\divide\StrW\unitlength
\advance \StrW-2
\StrH\ht112\divide\StrH\unitlength
\advance \StrH3
\hspace*{1\point}
\psline{c-c}(2,-2)(\StrW,\StrH)
\copy112
\hspace*{1\point}}

 \def \Neg#1{#1,\Sink}
 \def \Map #1-#2 {{#1},{#2}}
 \def \Plus #1+#2 {{#1}{+}{#2}}
 \def \Plus #1+#2 {{#1},{#2}}
 \def \NotUsedSymb{\nonconnectable}%{ `o}
 \def \NotUsed{\NotUsedSymb}
 \def \NotOcc{\varn}
 \def \SinkSymb{\psset{unit=.9\point,linewidth=.4\point%,linecolor=picolour
 }\hbox to 6\point{%\qdisk(2.75,2.75){2\point}
 \psline{c-c}(2,5)(4,5)
 \psline{c-c}(1,2.75)(5,2.75)
 \psline{c-c}(0,.5)(6,.5)
 }}
 \def \Sink{\SinkSymb}

\def \semcolour{}

\setbox144=\hbox{{\semcolour \leavevmode\raise1\point\hbox{${\lceil}\kern-3\point{\lceil}$}}}
\setbox145=\hbox{{\semcolour \raise1\point\hbox{${\rfloor}\kern-3\point{\rfloor}$}}}
 \def \SemMxi#1#2{\copy144{\lterm {#1} } \copy145
\setbox153=\hbox{$_{\semcolour #2}$}
\setbox154=\hbox{\scriptsize $\semcolour \cal M$}
\ifdim \wd154 > \wd153 {\copy153\kern-\wd153 \hbox{\raise5\point\hbox{\box154}}}
\else {\raise5\point\hbox{\copy154}\kern-\wd154 \box153}
\fi
}
 \def \SemM#1{\@ifnextchar{\bgroup}{\SemMxi{#1}}{\SemMxi{#1}{\xi}}}

\def \BPiSem{\Bang \PiSem}
\def \PiSemGen[#1] #2 {\omtrue \lefttop {\termcolour #1 } \righttop \kern-2\adjustablepoint \raise-3.75\adjustablepoint\hbox{\textsc{\scriptsize #2}}\kern0\adjustablepoint}

\def \PiSemOne[#1]{{\picolour \leftsem {\termcolour #1 } \rightsem } \kern2\point}
 \def \PiSemTwo[#1]<#2>{\lefttop {\termcolour #1 } \righttop\kern-.75\point_{\textsc{\scriptsize #2}} \kern0.5\point}
 \def \PiSem[#1]{\@ifnextchar<{\PiSemTwo[#1]}{\PiSemOne[{#1}]}}
% \def \PiFSem[#1]{\PiSemGen[{\Greencol #1}] f \picolour }
 \def \PiFSem[#1] #2 {{\semPi{\LTerm<{#1}>}<f>} \skp {#2} }

 \def \BPiFSem[#1]{\Bang \PiFSem[#1]}
 \def \PiRSem[#1]{{\PiSemGen[{#1}] s }} % used to be r
 \def \BPiRSem[#1]{\Bang \PiRSem[#1]}

% \def \PiSemL[#1]{\ifnextchar\bgroup{\Sem{\lterm {#1} }\kern-1\point\raise7\point\hbox{\tiny $`p$}\kern-2\point}{{\Sem{\lterm {#1} }}\picolour }}

\def \PiSemL[#1]{\ifnextchar\bgroup{\Sem{\lterm {#1} }\kern-1\point\raise7\point\hbox{\tiny $`p$}\kern-2\point}{{\PiSemGen [\lterm {#1} }] {`p} \picolour }}

 \def \PiNSem[#1]{\lefttop {\termcolour #1 } \righttop \kern-1\point_{\mysemcolour `p}\kern-3\point^{\textsc{\scriptsize n}} }
 \def \PiNSemL#1#2{\SemThree{#1}{#2}{\mbox{\mysemcolour \scriptsize $`p$}}^{\textsc{\scriptsize n}}}

 \def \PiVSem#1{\lefttop {\termcolour #1 } \righttop \kern-1\point_{\mysemcolour `p}\kern-3\point^{\textsc{\scriptsize v}} }
 \def \PiVSemL#1#2{\SemThree{#1}{#2}{\mbox{\mysemcolour \scriptsize $`p$}}^{\textsc{\scriptsize v}}}

% \def \piCut#1#2#3#4{{\picolour ( \piCutL{#1}{#2}{#3}{#4} ) \Choice ( \piCutR{#1}{#2}{#3}{#4} ) }}
 \def \piCutN#1#2#3#4{{\picolour \New {#2} ( {#1} \Par \Bang { \New {#3} ( \Eq{#2}={#3} \Par {#4} ) } ) }}
 \def \piCutV#1#2#3#4{{\picolour \New {#3} ( \Bang { \New {#2} ({#1} \Par \Eq{#2}={#3} ) } \Par {#4} ) }}
 \def \piCut#1#2#3#4{{\picolour \New {#2#3} ( \Bang {#1} \Par \Bang \Eq{#2}={#3} \Par \Bang {#4} ) }}
 \def \piCutLog#1#2#3#4{{\picolour \New {#2#3} ( #1 {} \Par \Eq{#2}={#3} \Par {} #4 ) }}
 \def \piCutL#1#2#3#4{{\picolour \New {#2#3} ( {#1} \Par \Bang { \Eq{#2}={#3} } \Par \Bang {#4} ) }}
 \def \piCutR#1#2#3#4{{\picolour \New {#2#3} ( \Bang {#1} \Par \Bang { \Eq{#2}={#3} } \Par {#4} ) }}
%
 \def \piCutLunfold#1#2#3#4{{\picolour \New {#2} ( {#1} \Par { \New {#3} ( \Eq{#2}={#3} \Par {#4} ) } \Par \Bang { \ldots } ) }}
 \def \piCutRunfold#1#2#3#4{{\picolour \New {#3} ( \Bang { \ldots } \Par { \New {#2} ({#1} \Par \Eq{#2}={#3} ) } \Par {#4} ) }}
%
% \def \piCutdl#1#2#3#4{{\picolour ( \piCutL{#1}{#2}{#3}{#4} ) \qquad \hfill \Choice ~~ \\ \hfill ( \piCutR{#1}{#2}{#3}{#4} )}}
 \def \piCap#1#2{{\picolour \In {#1} (\Arg) . \Out {#2} <\Arg> }}
%
 \def \piImpAlt #1 #2 [#3] #4 #5 {{\picolour
 \New {#2#4} ({ \Bang{ #1 } \Par
 \In {#3} (\Map \varv-{\vard} ) .
 	({ \Bang { \Eq{#2}={\varv} } \Par \Bang { \Eq{\vard}={#4} } })
	\Par \Bang{#5}
	})
}}
%
 \def \piImp#1#2#3#4#5{{\picolour \In {#3} (\Map \vars-{\vard} ) . ({
	\New {#2} ( \Bang{ #1 } \Par \Bang { \Eq{#2}={\vars} } )
 \Par
	\New {#4} ( \Bang { \Eq{\vard}={#4} } \Par \Bang{#5} )
 })%
}}
%
 \def \piImpVars#1#2#3#4#5#6#7{{\picolour \In {#3} (\Map #6-#7 ) . \New {#2} ( \Bang{ #1 \Par \Eq{#2}={#6} } ) \Par \New {#4} ( \Bang { \Eq{#7}={#4} \Par #5 } ) }}
%
 \def \piImpdl#1#2#3#4#5{ \In {#3} (\Map \vars-{\vard} ) . {} (
	\New {#2} { \Bang ( {#1} \Par \Bang { \Eq{#2}={\vars} } ) }
 \Par
{} \quad \\[-2\point] \quad \hfill 
	\New {#4} ( \Bang { \Eq{\vard}={#4} } \Par \Bang{#5} )
 )
}
 \def \piExp#1#2#3#4{\New {#1#3} ( \Bang #2 \Par \Out {#4} <{\Map {#1}-{#3} }> ) }

 \def \piInvL#1#2#3{{\picolour \In {#1} (z,\NotOcc) . ( \New {#3} ({ \Bang{#2} \Par \BEq{#3}=z ) }) }}
 \def \piInvR#1#2#3{{\picolour \New {#1} ( \Bang{#2} \Par \Out{#3} <\Neg{#1}N> ) }}
 \def \piHInvL#1#2#3{{\picolour \In {#1} (z) . ( \New {#3} ({ \Bang{#2} \Par \BEq{#3}=z ) }) }}
 \def \piHInvR#1#2#3{{\picolour \New {#1} ( \Bang{#2} \Par \Out{#3} <#1> ) }}
 \def \piAndLL#1#2#3#4{{\picolour \In {#1} (v,\NotOcc) . ({ \New {#2} ( \BEq v=#2 \Par \Bang {#4} ) }) }}
 \def \piAndLR#1#2#3#4{{\picolour \In {#1} (\NotOcc,v) . ({ \New {#3} ( \BEq v=#3 \Par \Bang {#4} ) }) }}
 \def \piAndR#1#2#3#4{%
 {\picolour \In {#1} (#2,v) . (\Eq v={#3} ) \Par \Bang {#4} }}
 \def \piAndL#1#2#3#4{{\picolour \In {#1} (#2,#3) . \Bang {#4} }}
 \def \piAndR#1#2#3#4#5{{\picolour \New {#2},{#4} (\Bang{#1} \Choice \Bang{#3} \Par \Out{#5} <{#2,#4}> ) }}
% \def \piOrL#1#2#3#4#5{{\picolour \In {#1} (\Plus {\vara}+{\varb} ) . (\New {#2} ( \Bang{\Eq{\vara}={#2} } \Par \Bang{#3} ) \Choice \New {#4} ( \Bang{\Eq{\varb}={#4} } \Par \Bang{#5} ) ) }}
 \def \piOrL#1#2#3#4#5{{\picolour
 	\In {#1} (\Plus {\vara}+{\varb} ) .
		(\New {#2} ( \Bang{\Eq{\vara}={#2} } \Par \Bang{#3} )
		\Choice
		\New {#4} ( \Bang{\Eq{\varb}={#4} } \Par \Bang{#5} ) )
}}
 \def \piFOrL#1#2#3#4#5{{\picolour
 \New {#2#4} ({ \Bang{#3} \Par
		\In {#1} (\Plus {\vara}+{\varb} ) . ( \Bang{\Eq{\vara}={#2} }
		\Par
		\Bang{\Eq{\varb}={#4} } ) \Par \Bang{#5}
	})
}}
 \def \piOrRL#1#2#3#4{{\picolour \New #2 ( \Bang{#1} \Par \Out{#4} < \Plus #2+{#3} >) }}
 \def \piOrRR#1#2#3#4{{\picolour \New #3 ( \Bang{#1} \Par \Out{#4} < \Plus #2+#3 >) }}
 \def \piOrRP#1#2#3#4{{\picolour \New #2#3 ( #1 \Par \Out{#4} < \Plus \Bang{#2}+\Bang{#3} >) }}


 \def \Picut #1 #2 + #3 #4 { \piCut{#1}{#2}{#3}{#4} }
 \def \PicutLog #1 #2 + #3 #4 { \piCutLog{#1}{#2}{#3}{#4} }
 \def \Picutunfold #1 #2 + #3 #4 { \piCutLunfold {#1}{#2}{#3}{#4} \Choice \piCutRunfold {#1}{#2}{#3}{#4} }
 \def \Picutdl #1 #2 + #3 #4 {
	(\nu {#2#3}) \, ( \Bang {#1} \Par \Bang { \Eq{#2}={#3} } \Par {} \quad \\[-2\point] \dquad \hfill {\picolour \Bang {#4} )
} }
 \def \PicutAuxdl #1 #2 + #3 #4 {
	(\nu {#2#3}) \, ( \Bang {#1} \Par \Bang { \Eq{#2}={#3} } \Par {} \quad \\[-2\point] \dquad \hfill {\picolour {#4} )
} }
 \def \PicutLogdl #1 #2 + #3 #4 { {\picolour
	(\nu {#2#3}) \, ( {#1} \Par \Eq{#2}={#3} \Par {} } \\[-2\point] \quad \hfill {\picolour {#4} )
} }
 \def \PicutL #1 #2 + #3 #4 { \piCutL{#1}{#2}{#3}{#4} }
 \def \PicutR #1 #2 + #3 #4 { \piCutR{#1}{#2}{#3}{#4} }
%
 \def \PicutLunfold #1 #2 + #3 #4 { \piCutLunfold{#1}{#2}{#3}{#4} }
 \def \PicutRunfold #1 #2 + #3 #4 { \piCutRunfold{#1}{#2}{#3}{#4} }
%
 \def \Picaps<#1,#2>{ \piCap{#1}{#2} }
%
 \def \Piimp{\@ifnextchar({\PiimpVars}{\PiimpNormal}}%)
 \def \PiimpVars (#1,#2) #3 #4 [#5] #6 #7 { \piImpVars{#3}{#4}{#5}{#6}{#7}{#1}{#2} }
 \def \PiimpNormal #1 #2 [#3] #4 #5 { \piImp{#1}{#2}{#3}{#4}{#5} }
 \def \Piimpdl #1 #2 [#3] #4 #5 { \piImpdl{#1}{#2}{#3}{#4}{#5} }
%
 \def \Piexp #1 #2 #3 . #4 {\piExp{#1}{#2}{#3}{#4} }
%
 \def \PiinvL #1 . #2 #3 {\piInvL{#1}{#2}{#3}}
 \def \PiinvR #1 #2 . #3 {\piInvR{#1}{#2}{#3}}
%
 \def \PiprojLR #1 . < #2 , #3 > #4 {\piAndL{#1}{#2}{#3}{#4}}
 \def \PiprojLaux #1 . < #2 , {\@ifnextchar{o}{\PiprojL #1 . < #2 , }{\PiprojLR #1 . < #2 , }}
 \def \Piproj #1 . < {\@ifnextchar{o}{\PiprojR {#1} . < }{\PiprojLaux {#1} . < }}
 \def \PiprojL #1 . < #2 , #3 > #4 {\piAndLL{#1}{#2}{\NotUsed}{#4}}
 \def \PiprojR #1 . < #2 , #3 > #4 {\piAndLR{#1}{\NotUsed}{#3}{#4}}
%
 \def \Pipair < #1 #2 , #3 #4 > . #5 {\piAndR{#1}{#2}{#3}{#4}{#5}}
 \def \PiinP #1 < {\@ifnextchar{o}{\PiinR {#1} < }{\PiinLaux {#1} < }}
 \def \PiinLaux #1 < #2 | {\@ifnextchar{o}{\PiinL #1 < #2 | }{\PiorRP #1 < #2 | }}
 \def \PiinL #1 < #2 | #3 > . #4 {\piOrRL{#1}{#2}{\varn}{#4}}
 \def \PiinR #1 < #2 | #3 > . #4 {\piOrRR{#1}{\varn}{#3}{#4}}
 \def \PiorRP #1 < #2 | #3 > . #4 {\piOrRP{#1}{#2}{#3}{#4}}
 \def \Pichoice #1 . < #2 #3 | #4 #5 > {\piOrL{#1}{#2}{#3}{#4}{#5}}

 \def \SHcaps<#1,#2>{\PiHSem[ \Cap{#1}{#2} ]}
 \def \SHexp #1 #2 #3 . #4 {\PiHSem[ \Exp{#1}{#2}{#3}{#4} ]}
 \def \SHimp #1 #2 [#3] #4 #5 {\PiHSem[ \Med{#1}{#2}{#3}{#4}{#5} ]}
 \def \SHcut #1 #2 + #3 #4 {\PiHSem[ \Cut{#1}{#2}{#3}{#4} ]}
 \def \SHcutLog #1 #2 + #3 #4 {\PiHSem[ \CutLog{#1}{#2}{#3}{#4} ]}
 \def \SHcutL #1 #2 + #3 #4 {\PiHSem[ \CutL{#1}{#2}{#3}{#4} ]}
 \def \SHcutR #1 #2 + #3 #4 {\PiHSem[ \CutR{#1}{#2}{#3}{#4} ]}
 \def \SHinvL #1 . #2 #3 {\PiHSem[ \InvLterm{#1}{#2}{#3} ]}
 \def \SHinvR #1 #2 . #3 {\PiHSem[ \InvRterm{#1}{#2}{#3} ]}
 \def \SHproj #1 . < #2 , #3 > #4 {\PiHSem[ \proj #1 . < #2 , #3 > #4 ]}
 \def \SHprojL #1 . < #2 , #3 > #4 {\PiHSem[ \AndLL{#1}{#2}{\NotUsed}{#4} ]}
 \def \SHprojR #1 . < #2 , #3 > #4 {\PiHSem[ \AndLR{#1}{\NotUsed}{#3}{#4} ]}
 \def \SHpair < #1 #2 , #3 #4 > . #5 {\PiHSem[ \AndR{#1}{#2}{#3}{#4}{#5} ]}
 \def \SHinL #1 < #2 | #3 > . #4 {\PiHSem[ \OrRL{#1}{#2}{\NotUsed}{#4} ]}
 \def \SHinR #1 < #2 | #3 > . #4 {\PiHSem[ \OrRR{#1}{\NotUsed}{#3}{#4} ]}
 \def \SHinP #1 < #2 | #3 > . #4 {\PiHSem[ \OrRP{#1}{#2}{#3}{#4} ]}
 \def \SHchoice #1 . < #2 #3 | #4 #5 > {\PiHSem[ \OrL{#1}{#2}{#3}{#4}{#5} ]}

 \def \SFcaps<#1,#2>{\PiFSem[ \Cap{#1}{#2} ]}
 \def \SFexp #1 #2 #3 . #4 {\PiFSem[ \Exp{#1}{#2}{#3}{#4} ]}
 \def \SFimp #1 #2 [#3] #4 #5 {\PiFSem[ \Med{#1}{#2}{#3}{#4}{#5} ]}
 \def \SFcut #1 #2 + #3 #4 {\PiFSem[ \Cut{#1}{#2}{#3}{#4} ]}
 \def \SFcutLog #1 #2 + #3 #4 {\PiFSem[ \CutLog{#1}{#2}{#3}{#4} ]}
 \def \SFcutL #1 #2 + #3 #4 {\PiFSem[ \CutL{#1}{#2}{#3}{#4} ]}
 \def \SFcutR #1 #2 + #3 #4 {\PiFSem[ \CutR{#1}{#2}{#3}{#4} ]}
 \def \SFinvL #1 . #2 #3 {\PiFSem[ \InvLterm{#1}{#2}{#3} ]}
 \def \SFinvR #1 #2 . #3 {\PiFSem[ \InvRterm{#1}{#2}{#3} ]}
 \def \SFproj #1 . < #2 , #3 > #4 {\PiFSem[ \proj #1 . < #2 , #3 > #4 ]}
 \def \SFprojL #1 . < #2 , #3 > #4 {\PiFSem[ \AndLL{#1}{#2}{\NotUsed}{#4} ]}
 \def \SFprojR #1 . < #2 , #3 > #4 {\PiFSem[ \AndLR{#1}{\NotUsed}{#3}{#4} ]}
 \def \SFpair < #1 #2 , #3 #4 > . #5 {\PiFSem[ \AndR{#1}{#2}{#3}{#4}{#5} ]}
 \def \SFinL #1 < #2 | #3 > . #4 {\PiFSem[ \OrRL{#1}{#2}{\NotUsed}{#4} ]}
 \def \SFinR #1 < #2 | #3 > . #4 {\PiFSem[ \OrRR{#1}{\NotUsed}{#3}{#4} ]}
 \def \SFinP #1 < #2 | #3 > . #4 {\PiFSem[ \OrRP{#1}{#2}{#3}{#4} ]}
 \def \SFchoice #1 . < #2 #3 | #4 #5 > {\PiFSem[ \OrL{#1}{#2}{#3}{#4}{#5} ]}

 \def \Scaps<#1,#2>{\PiSem[ \Cap{#1}{#2} ]}
 \def \Sexp #1 #2 #3 . #4 {\PiSem[ \Exp{#1}{#2}{#3}{#4} ]}
 \def \Simp #1 #2 [#3] #4 #5 {\PiSem[ \Med{#1}{#2}{#3}{#4}{#5} ]}
 \def \Scut #1 #2 + #3 #4 {\PiSem[ \Cut{#1}{#2}{#3}{#4} ]}
 \def \ScutLog #1 #2 + #3 #4 {\PiSem[ \CutLog{#1}{#2}{#3}{#4} ]}
 \def \ScutL #1 #2 + #3 #4 {\PiSem[ \CutL{#1}{#2}{#3}{#4} ]}
 \def \ScutR #1 #2 + #3 #4 {\PiSem[ \CutR{#1}{#2}{#3}{#4} ]}
 \def \SinvL #1 . #2 #3 {\PiSem[ \InvLterm{#1}{#2}{#3} ]}
 \def \SinvR #1 #2 . #3 {\PiSem[ \InvRterm{#1}{#2}{#3} ]}
 \def \Sproj #1 . < #2 , #3 > #4 {\PiSem[ \proj #1 . < #2 , #3 > #4 ]}
 \def \SprojL #1 . < #2 , #3 > #4 {\PiSem[ \AndLL{#1}{#2}{\NotUsed}{#4} ]}
 \def \SprojR #1 . < #2 , #3 > #4 {\PiSem[ \AndLR{#1}{\NotUsed}{#3}{#4} ]}
 \def \Spair < #1 #2 , #3 #4 > . #5 {\PiSem[ \AndR{#1}{#2}{#3}{#4}{#5} ]}
 \def \SinL #1 < #2 | #3 > . #4 {\PiSem[ \OrRL{#1}{#2}{\NotUsed}{#4} ]}
 \def \SinR #1 < #2 | #3 > . #4 {\PiSem[ \OrRR{#1}{\NotUsed}{#3}{#4} ]}
 \def \SinP #1 < #2 | #3 > . #4 {\PiSem[ \OrRP{#1}{#2}{#3}{#4} ]}
 \def \Schoice #1 . < #2 #3 | #4 #5 > {\PiSem[ \OrL{#1}{#2}{#3}{#4}{#5} ]}

 \def \NScaps<#1,#2>{\PiNSem[ \Cap{#1}{#2} ]}
 \def \NSexp #1 #2 #3 . #4 {\PiNSem[ \Exp{#1}{#2}{#3}{#4} ]}
 \def \NSimp #1 #2 [#3] #4 #5 {\PiNSem[ \Med{#1}{#2}{#3}{#4}{#5} ]}
 \def \NScut #1 #2 + #3 #4 {\PiNSem[ \Cut{#1}{#2}{#3}{#4} ]}
 \def \NScutL #1 #2 + #3 #4 {\PiNSem[ \CutL{#1}{#2}{#3}{#4} ]}
 \def \NScutR #1 #2 + #3 #4 {\PiNSem[ \CutR{#1}{#2}{#3}{#4} ]}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 \def \SFcaps<#1,#2>{\PiFSem[ \Cap{#1}{#2} ]}
 \def \SFexp #1 #2 #3 . #4 {\PiFSem[ \Exp{#1}{#2}{#3}{#4} ]}
 \def \SFimp #1 #2 [#3] #4 #5 {\PiFSem[ \Med{#1}{#2}{#3}{#4}{#5} ]}
 \def \SFcut #1 #2 + #3 #4 {\PiFSem[ \Cut{#1}{#2}{#3}{#4} ]}
 \def \SFcutLog #1 #2 + #3 #4 {\PiFSem[ \CutLog{#1}{#2}{#3}{#4} ]}
 \def \SFcutL #1 #2 + #3 #4 {\PiFSem[ \CutL{#1}{#2}{#3}{#4} ]}
 \def \SFcutR #1 #2 + #3 #4 {\PiFSem[ \CutR{#1}{#2}{#3}{#4} ]}

\def \PiHcaps<#1,#2>{ \In {#1} (w) . \Out {#2} <w> }
\def \PiHexp #1 #2 #3 . #4 {{\picolour \NewA #1#3 ( \Bang {#2} \Par \Out {#4} <{\Map {#1}-{#3} }> ) }}

\def \PiHimp #1 #2 [#3] #4 #5 {{\picolour \In {#3} (\Map {#2}-{#4} ) . ({ \Bang {#1} \Par \Bang {#5} }) }}
 \def \PiHImpdl #1 #2 [#3] #4 #5 {{\picolour \In {#3} (\Map {#2}-{#4} ) . {} (
	\New {#2} { \Bang ( {#1} ) } 			\Par
{} \quad } \\[-2\point] \quad \hfill {\picolour
	\New {#4} \Bang ( {#5} )				)}}
%
\def \PiHcut #1 #2 + #3 #4 {{\picolour \New {#3} ({ \Bang {#1[{#3}/{#2}]} \Par \Bang{#4} }) }}
\def \PiHcutS #1 #2 + #3 #4 {\piHCutS{#1}{#2}{#3}{#4}}
\def \piHCutS#1#2#3#4{{\picolour \New {#3} ({ \Bang{#1} \Par \Bang{#4} }) }}
%\def \piHcutLog#1#2#3#4{{\picolour \New {#3} ( {#1[{#3}/{#2}]} \Par {#4} ) }}
\def \PiHcutLog #1 #2 + #3 #4 {{\picolour \New {#3} ({ {#1[{#3}/{#2}]} \Par {#4} }) }}
\def \PiHcutLogS #1 #2 + #3 #4 {\piHCutLogS{#1}{#2}{#3}{#4}}
\def \piHCutLogS#1#2#3#4{{\picolour \New {#3} ({ {#1} \Par {#4} }) }}
\def \PiHcutdl #1 #2 + #3 #4 {
	(\nu {#2}) \, ( \Bang {#1[#3/#2]} \Par \quad \\[-2\point] \dquad \hfill {\picolour \Bang {#4} ) } }
\def \PiHcutdlS #1 #2 + #3 #4 {
	(\nu {#2}) \, ( \Bang {#1} \Par \quad \\[-2\point] \dquad \hfill {\picolour \Bang {#4} ) } }
%
 \def \PiHinvL #1 . #2 #3 {{\picolour \In {#1} (#3) . \Bang{#2} }}
 \def \PiHinvR #1 #2 . #3 {{\picolour \New {#1} ( \Bang{#2} \Par \Out{#3} <{#1}> ) }}

\def \indentstep{~%\theindent
\stepcounter{indent}\ifnum\theindent=1\dquad \else\ifnum\theindent=2\qquad \else\ifnum\theindent=3\tquad\fi\fi\fi}

 \def \PiFcut #1 #2 + #3 #4 {\NewA #2#3 ( \Bang #1 \Par \Bang \Eq{#2}={#3} \Par \Bang #4 )}
 \def \PiFcutX #1 #2 + #3 #4 {\NewA #2#3 ( \Bang {#1} \Par \Bang \EqX{#2}={#3} \Par \Bang {#4} )}
 \def \PiFcutLog #1 #2 + #3 #4 {\NewA #2#3 ( #1 \Par \Eq{#2}={#3} \Par #4 ) }
 \def \PiFcutLogX #1 #2 + #3 #4 {\NewA #2#3 ( #1 \Par \EqX{#2}={#3} \Par #4 ) }
 \def \PiFcutLogdl #1 #2 + #3 #4 {\NewA #2#3 ( #1 \Par \Eq{#2}={#3} \Par \\[-1\point] \indentstep %\hfill
 #4 )\addtocounter{indent}{-1}}
 \def \PiFcutLogXdl #1 #2 + #3 #4 {\NewA #2#3 ( #1 \Par \EqX{#2}={#3} \Par \\[-1\point] \indentstep %\hfill
 #4 )\addtocounter{indent}{-1}}
 \def \PiFcutdl #1 #2 + #3 #4 {\NewA #2#3 ( \Bang #1 \Par \Bang \Eq{#2}={#3} \Par \\ \indentstep %\hfill
 \Bang #4 )\addtocounter{indent}{-1}}
 \def \PiFcutXdl #1 #2 + #3 #4 {\NewA #2#3 ( \Bang #1 \Par \Bang \EqX{#2}={#3} \Par \\ \indentstep %\hfill
 \Bang #4 )\addtocounter{indent}{-1}}
 \def \PiFcutdlMC #1 #2 + #3 #4 {\NewA #2#3 ( \Bang #1 \Par \Bang \Eq{#2}={#3} \Par \quad \multicolumn{3}{r}{ \quad \Bang #4 )}}

 \def \PiFcutL #1 #2 + #3 #4 {\NewA #2#3 ( \Bang #1 \Par \Bang { \Eq{#2}={#3} } \Par \Bang #4 ) }
 \def \PiFcutR #1 #2 + #3 #4 {\NewA #2#3 ( \Bang #1 \Par \Bang { \Eq{#2}={#3} } \Par \Bang #4 ) }
% \def \PicutLunfold #1 #2 + #3 #4 { \piCutLunfold{#1}{#2}{#3}{#4} }
% \def \PicutRunfold #1 #2 + #3 #4 { \piCutRunfold{#1}{#2}{#3}{#4} }
%
 \def \PiFcaps<#1,#2>{ \piFCap{#1}{#2} }
%
 \def \PiFimp{\@ifnextchar({\PiFimpVars}{\PiFimpNormal}}%)
 \def \PiFimpVars (#1,#2) #3 #4 [#5] #6 #7 { \piFImpVars{#3}{#4}{#5}{#6}{#7}{#1}{#2} }
 \def \PiFimpNormal #1 #2 [#3] #4 #5 {
 	\NewA #2#4 ( \Bang #1 \Par \In {#3} (v,d) . ({ \BEq{#2}=v \Par \BEq d={#4} }) \Par \Bang #5 ) }
 \def \PiFimpdl #1 #2 [#3] #4 #5 {\NewA #2#4 ( \Bang #1 \Par {#3} (v,d) \, . \, ( \BEq{#2}=v \Par \BEq d={#4} ) \Par ~ \\[-2\point] \indentstep
 \Bang #5 ) \addtocounter{indent}{-1}}
 \def \PiFimpedl #1 #2 [#3] #4 #5 {\NewA #2#4 ( \Bang #1 \Par ~ \\ \indentstep {#3} (v,d) \, . \, ( \BEq{#2}=v \Par \BEq d={#4} ) \Par \Bang #5 ) \addtocounter{indent}{-1}}
 \def \PiFimpeWdl #1 #2 [#3] #4 #5 {W\multicolumn{3}{l}{\NewA #2#4 ( \Bang #1 \Par ~ } \\ \indentstep {#3} (v,d) \, . \, ( \BEq{#2}=v \Par \BEq d={#4} ) \Par \Bang #5 ) \addtocounter{indent}{-1}}
%
 \def \PiFexp #1 #2 #3 . #4 {\NewA #1#3 ( \Bang {#2} \Par \Out {#4} <{\Map {#1}-{#3} }> ) }


 \def \PiFinvL #1 . #2 #3 {\New {#3} ({ \Bang{#2} \Par \In {#1} (z) . ( \BEq{#3}=z ) }) }
 \def \PiFinvR #1 #2 . #3 {\New {#1} ( \Bang{#2} \Par \Out{#3} <#1> ) }

 \def \piFAndLR#1#2#3#4{\New {#3} ({ \In {#1} (\NotOcc,v) . ( \BEq v=#3 ) \Par \Bang #4 }) }


 \def \PiFprojLR #1 . < #2 , #3 > #4 {\New {#2} ({ \In {#1} (v,\NotOcc) . ( \BEq v=#2 ) \Par \Bang #4 }) }
 \def \PiFprojLaux #1 . < #2 , {\@ifnextchar{o}{\PiFprojL #1 . < #2 , }{\PiFprojLR #1 . < #2 , }}
 \def \PiFproj #1 . < {\@ifnextchar{o}{\PiFprojR {#1} . < }{\PiFprojLaux {#1} . < }}
 \def \PiFprojL #1 . < #2 , #3 > #4 {\piFAndLL{#1}{#2}{\NotUsed}{#4}}
 \def \PiFprojR #1 . < #2 , #3 > #4 {\piFAndLR{#1}{\NotUsed}{#3}{#4}}

 \def \PiFpair < #1 #2 , #3 #4 > . #5 {\New {#2},{#4} (\Bang{#1} \Choice \Bang{#3} \Par \Out{#5} <{#2,#4}> ) }
 \def \PiFinP #1 < {\@ifnextchar{o}{\PiFinR {#1} < }{\PiFinLaux {#1} < }}
 \def \PiFinLaux #1 < #2 | {\@ifnextchar{o}{\PiFinL #1 < #2 | }{\PiForRP #1 < #2 | }}
 \def \PiFinL #1 < #2 | #3 > . #4 {\piFOrRL{#1}{#2}{\Sink}{#4}}
 \def \PiFinR #1 < #2 | #3 > . #4 {\piFOrRR{#1}{\Sink}{#3}{#4}}
 \def \PiForRP #1 < #2 | #3 > . #4 {\piFOrRP{#1}{#2}{#3}{#4}}
 \def \PiFchoice #1 . < #2 #3 | #4 #5 > {\piFOrL{#1}{#2}{#3}{#4}{#5}}

% \def \piFAndL#1#2#3#4{{\picolour \In {#1} (#2,#3) . \Bang {#4} }}
 \def \piFOrL#1#2#3#4#5{{\picolour
 \New {#2#4} ({ \Bang{#3} \Par
		\In {#1} (\Plus {\vara}+{\varb} ) . ( \Bang{\Eq{\vara}={#2} }
		\Choice
		\Bang{\Eq{\varb}={#4} } ) \Par \Bang{#5}
	})
}}
 \def \piFOrRL#1#2#3#4{{\picolour \New #2 ( \Bang{#1} \Par \Out{#4} < \Plus #2+{#3} >) }}
 \def \piFOrRR#1#2#3#4{{\picolour \New #3 ( \Bang{#1} \Par \Out{#4} < \Plus #2+#3 >) }}
 \def \piFOrRP#1#2#3#4{{\picolour \New #2#3 ( #1 \Par \Out{#4} < \Plus \Bang{#2}+\Bang{#3} >) }}


 \def \piFCutN#1#2#3#4{{\picolour \NewA #2 ( {#1} \Par \Bang { \NewA #3 ( \Eq{#2}={#3} \Par {#4} ) } ) }}
 \def \piFCutV#1#2#3#4{{\picolour \NewA #3 ( \Bang { \NewA #2 ({#1} \Par \Eq{#2}={#3} ) } \Par {#4} ) }}
%
 \def \piFCutL{\piFCut}
 \def \piFCutR{\piFCut}
%
 \def \piFCutLunfold#1#2#3#4{{\picolour \NewA #2 ( {#1} \Par { \NewA #3 ( \Eq{#2}={#3} \Par {#4} ) } \Par \Bang { \ldots } ) }}
%
 \def \piFCutRunfold#1#2#3#4{{\picolour \NewA #3 ( \Bang { \ldots } \Par { \NewA #2 ({#1} \Par \Eq{#2}={#3} ) } \Par {#4} ) }}
%
 \def \piFCap#1#2{{\picolour \In {#1} (\Arg) . \Out {#2} <\Arg> }}
%
\def \LSynCellS #1 [#2] #3 { \qskp \BEq#1 = {\Eq[#2] = #3 } \qskp }
\def \LSynCell #1 [#2] #3 { \picolour \In {#2} (\Map v-d ) . ({ \BEq{#1}=v \Par \Eq d={#3} }) }
\def \SynCell #1 [#2] #3 {\picolour \In {#2} (\Map v-d ) . ({ \BEq{#1}=v \Par \BEq d={#3} }) }
%
 \def \piFImpAlt #1 #2 [#3] #4 #5 {{\picolour
 \NewA #2#4 ( \Bang{ #1 } \Par
 \In {#3} (\Map \varv-{\vard} ) .
 	({ \Bang { \Eq{#2}={\varv} } \Par \Bang { \Eq{\vard}={#4} } })
	\Par \Bang{#5}
	)
}}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Replicative encoding
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 \def \SRcaps<#1,#2>{\PiRSem[ \Cap{#1}{#2} ]}
 \def \SRexp #1 #2 #3 . #4 {\PiRSem[ \Exp{#1}{#2}{#3}{#4} ]}
 \def \SRimp #1 #2 [#3] #4 #5 {\PiRSem[ \Med{#1}{#2}{#3}{#4}{#5} ]}
 \def \SRcut #1 #2 + #3 #4 {\PiRSem[ \Cut{#1}{#2}{#3}{#4} ]}
 \def \SRcutLog #1 #2 + #3 #4 {\PiRSem[ \CutLog{#1}{#2}{#3}{#4} ]}
 \def \SRcutL #1 #2 + #3 #4 {\PiRSem[ \CutL{#1}{#2}{#3}{#4} ]}
 \def \SRcutR #1 #2 + #3 #4 {\PiRSem[ \CutR{#1}{#2}{#3}{#4} ]}
 \def \SRinvL #1 . #2 #3 {\PiRSem[ \InvLterm{#1}{#2}{#3} ]}
 \def \SRinvR #1 #2 . #3 {\PiRSem[ \InvRterm{#1}{#2}{#3} ]}

 \def \PiRcut #1 #2 + #3 #4 { \piRCut{#1}{#2}{#3}{#4} }
 \def \PiRcutdl #1 #2 + #3 #4 {% {\picolour
	(\nu {#2#3}) \, ( #1 \Par \Bang { \Eq{#2}={#3} } \Par {} %}
	\\[-1.5\point] \tab \hfill %{\picolour
	#4 ) }%}
 \def \PiRcutdlMC #1 #2 + #3 #4 {%{\picolour
 	\NewA {#2#3} ( {#1} \Par \Bang \Eq{#2}={#3} \Par {} %} 
	\\[-1.5\point]
	\multicolumn{3}{r}{ \quad %{\picolour 
	#4 ) } } %}
%
 \def \PiRcutL #1 #2 + #3 #4 { \piRCutL{#1}{#2}{#3}{#4} }
 \def \PiRcutR #1 #2 + #3 #4 { \piRCutR{#1}{#2}{#3}{#4} }
%
 \def \PiRcaps<#1,#2>{ \piRCap{#1}{#2} }
%
 \def \PiRimp{\@ifnextchar({\PiRimpVars}{\PiRimpNormal}}%)
 \def \PiRimpVars (#1,#2) #3 #4 [#5] #6 #7 { \piRImpVars{#3}{#4}{#5}{#6}{#7}{#1}{#2} }
 \def \PiRimpNormal #1 #2 [#3] #4 #5 { \piRImp{#1}{#2}{#3}{#4}{#5} }
 \def \PiRimpdl #1 #2 [#3] #4 #5 { \piRImpdl{#1}{#2}{#3}{#4}{#5} }
%
 \def \PiRexp #1 #2 #3 . #4 { \piRExp{#1}{#2}{#3}{#4} }
 \def \PiRinvL #1 . #2 #3 {\piRInvL{#1}{#2}{#3}}
 \def \PiRinvR #1 #2 . #3 {\piRInvR{#1}{#2}{#3}}

 \def \piRCut#1#2#3#4{%{\picolour 
\NewA #2#3 ( {#1} \Par \Bang \Eq{#2}={#3} \Par #4 ) }%}
 \def \piRCutLog#1#2#3#4{%{\picolour 
\NewA #2#3 ( #1 \Par \Eq{#2}={#3} \Par #4 ) }%}
 \def \piRCutL{\piRCut}
 \def \piRCutR{\piRCut}
%
 \def \piRCutLunfold#1#2#3#4{%{\picolour 
\NewA #2 ( #1 \Par \NewA #3 ( \Eq{#2}={#3} \Par #4 ) \Par \Bang { \ldots } ) }%}
 \def \piRCutRunfold#1#2#3#4{%{\picolour 
\NewA #3 ( \Bang \ldots \Par { \NewA #2 ({#1} \Par \Eq{#2}={#3} ) } \Par #4 ) }%}
%
 \def \piRCap#1#2{%{\picolour 
\Bang \In {#1} (\Arg) . \Out {#2} <\Arg> }%}
%
 \def \piRImpAlt #1 #2 [#3] #4 #5 {%{\picolour
\NewA #2#4 ( #1 \Par
\In {#3} (\Map \varv-{\vard} ) . ( \Bang \Eq{#2}={\varv} \Par \Bang \Eq{\vard}={#4} )
	\Par #5 ) }%}
%
 \def \piRImp#1#2#3#4#5{%{\picolour
\NewA #2#4 ( #1 \Par \Bang \In {#3} (\vars,\vard) . ( \Bang \Eq{#2}={\vars} \Par \Bang \Eq{\vard}={#4} ) \Par #5 ) }%}
%
 \def \piRImpVars#1#2#3#4#5#6#7{%{\picolour 
\In {#3} (\Map #6-#7 ) . \New {#2} ( \Bang{#1} \Par \Eq{#2}={#6} ) \Par \New {#4} ( \Bang \Eq{#7}={#4} \Par #5 ) }%}
%
 \def \piRImpdl#1#2#3#4#5{%{\picolour
 	\NewA {#2#4} (
		#1 \Par {}
	%}
	 \\[-1.5\point] ~~~ \hfill %{\picolour
		\Bang \In {#3} (\varv,\vard) . ({ \Bang \Eq{#2}={\varv} \Par \Bang \Eq{\vard}={#4} })
		\Par #5 ) }%}
%
 \def \piRExp#1#2#3#4{%{\picolour 
\New {#1#3} ( {#2} \Par \Bang \Out {#4} <{\Map {#1}-{#3} }> ) }%}

 \def \piRInvL#1#2#3{%{\picolour 
\New {#3} ({ #2 \Par \Bang \In {#1} (z) . ( \BEq{#3}=z ) }) }%}
 \def \piRInvR#1#2#3{%{\picolour 
\New {#1} ( #2 \Par \Bang \Out{#3} <#1> ) }%}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def \Picell <#1,#2> {\New x,`a ( ) }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


 \def \black{}
 \def \TurnPi {\mathrel{{\vdash}\kern-3pt_{`p}}}
 \def \Pider #1 : #2 |- #3 { \def \stat##1##2{{\picolour ##1}{:}{\typecolour ##2}}%
{\picolour #1 }{~}{:}{~}{\typecolour #2} \TurnPi {\typecolour #3}}
 \def \derPi {\Pider}

 \def \ssk{\hspace*{.5\point}}
 \def \achan {{\picolour a}}%{\textit{\orange \textsf{a}\ssk}}
 \def \bchan {{\picolour b}}%{\textit{\orange \textsf{b}\ssk}}
 \def \chan {{\picolour c}}%{\textit{\orange \textsf{c}\ssk}}
 \def \dchan {{\picolour d}}%{\textit{\orange \textsf{d}\ssk}}
 \def \nchan {{\picolour n}}%{\textit{\orange \textsf{d}\ssk}}
 \def \vara {{\picolour a}}%{\textit{\orange \textsf{a}\ssk}}
 \def \varb {{\picolour b}}%{\textit{\orange \textsf{b}\ssk}}
 \def \varc {{\picolour c}}%{\textit{\orange \textsf{c}\ssk}}
 \def \vard {{\picolour d}}%{\textit{\orange \textsf{d}\ssk}}
 \def \vare {{\picolour e}}%{\textit{\orange \textsf{e}\ssk}}
 \def \varn {\textrm{\orange \textsf{\small ?}\ssk}}
 \def \vars {{\picolour v}}%{\textrm{\orange \textsf{\small s}\ssk}}
 \def \varv {{\picolour v}}%{\textit{\orange \textsf{v}\ssk}}
 \def \varw {{\picolour w}}%{\textit{\orange \textsf{w}\ssk}}
 \def \varx {{\picolour x}}%{\textit{\orange \textsf{x}\ssk}}
 \def \vary {{\picolour y}}%{\textit{\orange \textsf{y}\ssk}}
 \def \varz {{\picolour z}}%{\textit{\orange \textsf{z}\ssk}}

 \def \redPiBr(#1){\mathrel{\Red \arrow\kern-1\point_{`p}\,(#1)}}
 \def \redpi {\mathrel{\Red \arrow\kern-1\point_{`p}}}
 \def \redPi {\@ifnextchar({\redPiBr}{\redpi}} 
 \def \redLPi {\mathrel{\Red \arrow\kern-1\point_{\mbox{\scriptsize \sc l}`p}}}
 \def \redNPi {\mathrel{\Red \arrow\kern-1\point_{\mbox{\scriptsize \sc n}`p}}}
 \def \rtcredNPi {\mathrel{\Red \arrow^*\kern-1\point_{\mbox{\scriptsize \sc n}`p}}}
 \def \dredPi {\mathrel{\Red \arrow \kern-8\point\arrow\kern-1\point_{`p}}}
 \def \stopsats {\mathbin{\Red \downarrow}_{\Red \mbox{\scriptsize \sc s}}}
 \def \convergesLPi {\,{\raise1\point\hbox{\Red \small $\downarrow_{\mbox{\scriptsize \sc l}`p}$}}}
 \def \divergesLPi {\,{\raise1\point\hbox{\Red \small $\uparrow_{\mbox{\scriptsize \sc l}`p}$}}}
 \def \convergesNPi {\,{\raise1\point\hbox{\Red \small $\downarrow_{\mbox{\scriptsize \sc n}`p}$}}}
 \def \divergesNPi {\,{\raise1\point\hbox{\Red \small $\uparrow_{\mbox{\scriptsize \sc n}`p}$}}}
 \def \convergesPi {\,{\raise1\point\hbox{\Red \small $\downarrow_{`p}$}}}
 \def \divergesPi {\,{\raise1\point\hbox{\Red \small $\uparrow_{`p}$}}}

 \def \redPiLoc {\mathrel{{\geq}\kern-2\point\raise5\point\hbox{\scriptsize $`p$}}}
%
 \def \geqPi{\mathrel{{\geq}\kern-1\point_{`p}}}
 \def \redPiFull {\mathrel{\black \arrow\kern-1\point_{`p}^{\mbox{\,\scriptsize \sc f}}}}
 \def \tcredPi {\mathrel{\Red {\rightarrow}\kern-.5\point^{+}_{`p}}}
 \def \rtcredPi {\mathrel{\Red {\rightarrow}\kern-.5\point^{\ast}_{`p}}}
 \def \lredP {{_{`p}\kern-3pt\leftarrow}}
 \def \bisimilar{\bisimilarity}
 \def \bisim{\bisimilarity}
 \def \antibi{\mathrel{\Red {\succeq}\kern-3\point\raise5\point\hbox{\scriptsize $`p$}}}
 \def \bisimilarity{\mathrel{\Red \raise5\point\hbox{\scriptsize $`p$}\kern-3.5\point{\preceq}}}
 \def \sbisimilarity{\mathrel{{\sim}\kern-1\point_{`p}}}
 \def \sbisim{\sbisimilarity}

 \def \equivalent{\mathrel{\sim}}
 \def \equivCBr(#1){\mathrel{{\Red {\sim}_{\mbox{\scriptsize \sc c}}\,(#1)}}}
 \def \equivc{\mathrel{{\Red {\sim}_{\mbox{\scriptsize \sc c}}}}}
 \def \equivC {\@ifnextchar({\equivCBr}{\equivc}} 
 \def \equivGC{\mathrel{{\Red {\sim}_{\mbox{\scriptsize \sc gc}}}}}
 \def \equivR{\mathrel{{\sim}_{\mbox{\scriptsize \sc r}}}}
 \def \gtC{\mathrel{\picolour_{\mbox{\scriptsize \sf c}}\kern-1\point{\sqsupseteq}}}
% \def \gtA{\mathrel{\picolour_{\mbox{\scriptsize \sf c}}\kern-1\point{\cal A}}}
 \def \stC{\mathrel{{\sqsubseteq}_{\mbox{\scriptsize \sf c}}}}
 \def \dirappPi{\mathrel{\sqsubseteq_{`p}}}
 \def \stPi{\mathrel{\sqsubseteq_{`p}}}
 \def \Ctg{\mathrel{{\sqsubseteq}_{\mbox{\scriptsize \sf c}}}}
 \def \crC{\mathrel{\raise1\point\hbox{${\downarrow}_{\mbox{\scriptsize \sf c}}$}}}
 \def \shows{\mathop{{\Red \downarrow}}}
 \def \Shows{\mathop{{\Red \Downarrow}}}

 \def \dirappPi{\mathrel{{\sqsubseteq}_{`p}}}
 \def \SetAppPiBr(#1){\mbox{\sfbf A}(#1)}
 \def \SetAppPi{\@ifnextchar({\SetAppPiBr}{\mbox{\sfbf A}}}


 \def \sbired#1{%\rightarrow\kern-16\point
{\sim}\psset{unit=1\point,linewidth=0.4\point}%
\put(3,2.7){%
\psline{c-c}(-.5,0.05)(-4.1,0.05)
\psline{c-c}(-.5,-0.05)(-4.1,-0.05)
\pscurve{c-c}(0,0)(-.5,0.24)(-1,0.6)(-1.5,1.25)(-2,2.5)%
\pscurve{c-c}(0,0)(-.5,-0.24)(-1,-0.6)(-1.5,-1.25)(-2,-2.5)%
}\hspace*{4\point}_{#1}}

 \def \sbired#1{%\rightarrow\kern-16\point
{\sim}\psset{unit=1\point,linewidth=0.4\point}%
\put(3,2.7){%
\psline{c-c}(-.5,0.05)(-4.1,0.05)
\psline{c-c}(-.5,-0.05)(-4.1,-0.05)
\pscurve{c-c}(0,0)(-.5,0.24)(-1,0.6)(-1.5,1.25)(-2,2.5)%
\pscurve{c-c}(0,0)(-.5,-0.24)(-1,-0.6)(-1.5,-1.25)(-2,-2.5)%
}\hspace*{4\point}_{#1}}

% \def \sbired#1{\rightsquigarrow_{#1}}

\def \sbired#1{\psset{unit=1\point,linewidth=2\point,linecolor=white}
\setbox176=\hbox{$\sim$}
\setbox177=\hbox{$\rightarrow$}
\kern2\point\copy177\kern-\wd177
\psline{c-c}(0,2.5)(4.6,2.5)
\kern-.2\wd176
\copy176
\kern.4\wd176%\kern\wd177
_{#1}}

 \def \ourredPi {\mathrel{\sbired{`p}}}
 \def \rtcourredPi {\mathrel{\sbired{`p}^{\ast}}}
 \def \redequivC {\mathrel{\sbired{\mbox{\scriptsize \sc c}}}}
 \def \redequivR {\mathrel{\sbired{\mbox{\scriptsize \sc r}}}}
 \def \rtcredequivR {\mathrel{\sbired{\mbox{\scriptsize \sc r}}\kern-4\point^{*}}}
 \def \rtcredequivR {\mathrel{\sbired{\mbox{\scriptsize \sc r}}\kern-4\point^{*}}}

 \def \equivredPi {\mathrel{\rightsquigarrow_{\mbox{\scriptsize \sc r}}}}
 \def \redR{\equivredPi}
 \def \rtcredR{\mathrel{\rightsquigarrow^{*}_{\mbox{\scriptsize \sc r}}}}

 \def \CR{~{\downarrow}~}
 \def \CRP{~{\downarrow}_{`p}~}

 \def \CRP{\raise-0.5\point\hbox{\rotatebox{20}{$\downarrow$}}{\bisimilarity}\raise1.5\point\hbox{\rotatebox{-20}{$\downarrow$}}}

\newcommand{\redcompi}{(\textit{Pi Comm})}
\newcommand{\redpar}{(\textit{Par})}
\newcommand{\redres}{(\textit{Res})}
\newcommand{\redcong}{(\textit{Str})}

%\newcommand{\StrCon}{\,{\black \equiv}\,}
\newcommand{\StrCon}{\mathrel{\equiv}}
\newcommand{\congruent}{\Red\StrCon}
%\newcommand{\Rule}[2]{\displaystyle{\frac{#1}{#2}}}

\newcommand{\myoutput}[2]{\PiOverline{#1}\langle #2\rangle}
\newcommand{\interoutput}[2]{\PiOverline{#1}<#2>}
\newcommand{\myinput}[2]{#1<#2>}
%\newcommand{\subst}[2]{\{ #1/ #2 \} }
 \def \fn(#1){\textit{fn}(#1)}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 \def \operatorname#1{\mathop{\mathrm{#1}}\nolimits}

 \def \assign{:=}
\newcommand{\dueto}[1]{\textup{\textbf{<#1> }}}
\newcommand{\nin}{\not\in}
\newcommand{\tmem}[1]{{\em #1\/}}
\newcommand{\tmop}[1]{\operatorname{#1}}

 \def \C	{\textrm{\sf C}}	
 \def \cmd [#1] #2 {\green [{#1}] {#2}}
 \def \mterm #1 [#2] #3 {\green `m {#1} . [{#2}] {#3}}
 \def \mabs #1 . #2 {\green `m {#1} . {#2}}
 \def \labs #1 . #2 {\green `l {#1} . {#2}}
 \def \lmdelayexpanded #1{\labs {f} . {\app {f} {#1} } }
% \def \lmdelay #1{ \left(#1\right)^\star }
 \def \lmdelay #1{\setbox129=\hbox{$#1$}%
\ifdim\wd129<6pt #1^\star\else<#1>^\star\fi}
% \def \lmforce #1{ \left(#1\right)^- }
 \def \lmforce #1{ <#1>^- }

% \def \app #1 #2{<#1><#2>}
% \def \app #1 #2{\left(#1\,#2\right)}
 \def \app #1 #2 {\setbox129=\hbox{$#1$}%
\ifdim\wd129<15pt #1\,#2\else<#1>#2\fi}
 \def \appbr #1 #2{(#1\,#2)}
 \def \appdl #1 #2{\begin{array}[t]{l}#1\\\qquad #2\end{array}}
 \def \appii #1 #2 #3 {\left(#1\,#2\,#3\right)}

 \def \LMSemN#1{{\Greenn \,\lefttop #1 \righttop \kern-1\point_{\textsc{\scriptsize n}}\kern-2\point\raise7\point\hbox{\scriptsize $`m$}}}
 \def \LMSemNO#1{{\Greenn \,\lefttop #1 \righttop \kern-1\point_{\textsc{\scriptsize n}}\kern-2\point\raise5\point\hbox{\tiny $`W$}}}

 \def \LMSemN#1{\Sem{\termcolour #1}{\textsc{\mysemcolour \scriptsize n}}{\hbox{\mysemcolour \scriptsize $`m$}}}
 \def \LMSemNA#1{\Sem{#1}{\textsc{\mysemcolour \scriptsize n}}{\hbox{\mysemcolour \scriptsize $`m'$}}}

 \def \LMSemNA#1{\LMSemN{#1}'{\mysemcolour '}}
 \def \SemNA#1{\SemN{#1}'}

 \def \LMSemV#1{{\Greenn \,\lefttop #1 \righttop \kern-1\point_{\picolour \textsc{\scriptsize v}}\kern-2\point\raise7\point\hbox{\scriptsize $`m$}}}
 \def \LMSemVO#1{{\Greenn \,\lefttop #1 \righttop \kern-1\point_{\picolour \textsc{\scriptsize v}}\kern-2\point\raise5\point\hbox{\tiny $`W$}}}

 \def \LMSemVA#1{\LMSemV{#1}'}
 \def \SemVA#1{\SemV{#1}'}

 \def \internal#1 {}

 \def \delay{\textsl{delay}}
 \def \CMD{\textsl{cmd}}
 \def \force{\textsl{force}}
 \def \delay{\textsl{delay}}
 \def \CPS{\textsc{cps}}
% \def \Cmd{\textsc{Cmd}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newdimen \totalwidth

\newsavebox{\Newb}\newsavebox{\Newba}\newsavebox{\Newbb}\newsavebox{\Newbc}
\newsavebox{\Newc}\newsavebox{\Newca}\newsavebox{\Newcb}\newsavebox{\Newcc}
\newsavebox{\Newd}\newsavebox{\Newda}\newsavebox{\Newdb}\newsavebox{\Newdc}
\newsavebox{\Newg}
\newsavebox{\Newq}
\newsavebox{\Newr}
\newsavebox{\Newv}
\newsavebox{\Neww}
\newsavebox{\Newx}
\newsavebox{\Newy}
\newsavebox{\Newz}
\newsavebox{\ArgOne}\newsavebox{\ArgTwo}
\newsavebox{\ArgThree}\newsavebox{\ArgThreea}

\newcounter{indent} \setcounter{indent}0

\newcount\depth \SetCtr{\depth}{0}
\newcounter{indb} \setcounter{indb}{-1}
\def \newb{\ifnum\theindb=-1$b$\else \ifnum\theindb=0{$b$}\else${b}_{\theindb}$\fi\fi\stepcounter{indb}}
\def\bind{\ifnum \theindb=0{b}\else{b_{\theindb}}\fi}
\newcounter{indc} \setcounter{indc}{-1}
% \def \newc{\ifnum\theindc=-1{$c$}\else\ifnum\theindc=0{$c$}\else${c}_{\theindc}$\fi\fi\stepcounter{indc}}
\def \newc{\ifnum\theindc=-1{$c$}\else\ifnum\theindc=0{$c'$}\else${c}_{\theindc}$\fi\fi\stepcounter{indc}}
\def\cind{\ifnum \theindc=0{c}\else{c_{\theindc}}\fi}
\newcounter{indd} \setcounter{indd}0
 \def \newd{\ifnum\theindd=-1{$d$}\else \ifnum\theindd=0{$d'$}\else$d_{\theindd}$\fi\fi\stepcounter{indd}}
\newcounter{inde} \setcounter{inde}{-1}
 \def \newe{\ifnum\theinde=-1{$e$}\else\ifnum\theinde=0{$e'$}\else${e}_{\theinde}$\fi\fi\stepcounter{inde}}
\def\eind{\ifnum \theinde=0{e}\else{e_{\theinde}}\fi}
\newcounter{indg}\setcounter{indg}0
 \def \newg{\ifnum\theindg=0{$g$}\else$g_{\theindg}$\fi\stepcounter{indg}}
\newcounter{indq} \setcounter{indq}0
 \def \newq{\ifnum\theindq=0{$q$}\else$q_{\theindq}4\fi\stepcounter{indq}}
\newcounter{indr} \setcounter{indr}0
 \def \newr{\ifnum\theindr=0{$r$}\else$r_{\theindr}$\fi\stepcounter{indr}}
\newcounter{indv} \setcounter{indv}0
 \def \newv{\ifnum\theindv=0{$v$}\else$v_{\theindv}$\fi\stepcounter{indv}}
\newcounter{indw} \setcounter{indw}0
 \def \neww{\ifnum\theindw=-1{$w$}\else$w_{\theindw}$\fi\stepcounter{indw}}
\newcounter{indx} \setcounter{indx}0
 \def \newx{\ifnum\theindx=0{$x$}\else$x_{\theindx}$\fi\stepcounter{indx}}
\newcounter{indy} \setcounter{indy}0
 \def \newy{\ifnum\theindy=0{$y$}\else$y_{\theindy}$\fi\stepcounter{indy}}
\newcounter{indz} \setcounter{indz}0
 \def \newz{\ifnum\theindz=-1{$z$}\else \ifnum\theindz=0{$z$}\else$z_{\theindz}$\fi\fi\stepcounter{indz}}

 \def \resetvariables{%
\setcounter{indb}{-1}%
\setcounter{indc}{-1}%
\setcounter{indd}{0}%
\setcounter{inde}{-1}%
\setcounter{indg}{0}%
\setcounter{indq}{0}%
\setcounter{indr}{0}%
\setcounter{indv}{0}%
\setcounter{indw}{-1}%
\setcounter{indx}{0}%
\setcounter{indy}{0}%
\setcounter{indz}{0}%
}

 \def \NextLine{\\}%{ \resetvariables}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 \def \var #1 {#1}
 \def \abs #1 . #2 {`l{#1}.{#2}}
 \def \app #1 #2 {{#1}\,{#2}}

 \def \MilSemOne[#1]{\OldSem[\LTerm <{#1}>]\kern-1\point^{\mbox{\semcolour \scriptsize \textsc m}}}
 \def \MilSemPOne[#1]{\OldSem[\LTerm <#1>]^{\mbox{\scriptsize \textsc p}}\picolour }
 \def \MilSem[#1]{{\OldSem[#1]{\kern-1\point\raise4\point\hbox{\semcolour \scriptsize \textsc m}} }\,\picolour }

 \def \Milvar #1 #2 {\Out{#1} <#2>}
 \def \Milabs #1 . #2 #3 {\In {#3} (#1,w) . {#2} w }
 \def \Milapp #1 #2 #3 {\New c ({#1} c \Par {\New z ( \Out {c} <z,#3> . \MilSem[z:= \lterm {#2} ] ) } ) }
 \def \Milsub [#1 := #2] {\Bang \In {#1} (w) . {\MilTerm [#2] w } }

% \def \newname{u}
 \def \NMilSem [{\@ifnextchar{L}{\MilSemAbs [}{\@ifnextchar{A}{\MilSemApp [}{\MilSemVar[}}}%]%]%]%]
 \def \MilSemAbs[#1 . #2] #3 {Abs {\picolour {#3}<{#1}>{#3}(w). \NMilSem[{#2}] w }}
 \def \MilSemApp[#1 #2] #3 {App {\Red \New v (\NMilSem[{#1}] v \Par {\New z ( \Out {v} <z> \Out {v} <{#3}> . \MilSem[z:={#2}] ) } ) }}
 \def \MilSemVar[#1] #2 {Var {\Green \Out {#1} <#2> }}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 \def \SMilTerm [#1] #2 {\piterm {\MilSem [\LTerm<#1>] {#2} } }

 \def \MilTerm [#1] #2 {\MilTermRec[#1] {#2} \resetvariables}

 \def \MilTermRec [%]
	{\@ifnextchar l{\MilTermAbs[}%]
	{\@ifnextchar a{\MilTermApp[}%]
	{\@ifnextchar X{\MilTermXpp[}%]
	{\@ifnextchar v{\MilTermVar[}%]
	{\@ifnextchar s{\MilTermsub[}%]
	{\@ifnextchar S{\MilTermSub[}%]
	{\@ifnextchar ({\MilTermBr[}%]
	{\MilTermAux[}%]
}}}}}}}

 \def \MilTermApp[a #1 #2] #3 {%
%\newc\newc
\setbox101=\hbox{\newc}\global\setbox105=\hbox{\newz}%
\setbox100=\hbox{$\NewA \copy101 (\MilTermRec [#1] {\copy101} \Par {} $}%
\global \setbox109=\hbox{$\NewA \copy105 ( \Out {\copy101} <\copy105> . \Out
{\box101} <{#3}> . % {\box105} := {#2} %
\MilSub [{\box105} := {#2}]
% \MilSemOne [S {\box105} := M]%  {\LTerm<{#2}>}
) ) $}
\totalwidth\wd100\advance\totalwidth\wd109
\ifdim\totalwidth>.9\textwidth
	{\ifdim\wd100>.45\textwidth
		\box100 ~ \\[-2pt] \hfill \box109
	\else	\box100 \hfill \\[-2pt] ~ \box109\fi}
\else \box100 \box109\fi }

 \def \MilTermXpp[X #1 #2] #3 {%
\setbox101=\hbox{\newc}%
\setbox104=\hbox{\newz}%
\setbox100=\hbox{{\picolour $\NewA \copy101 (\MilTermRec [#1] {\copy101} \Par {} $}}%
\global \setbox109=\hbox{{\picolour $\NewA \copy104 ( \Out {\copy101} <\copy104> . \Out {\copy101} <{#3}> . \MilSubX [\copy104 := #2] ) ) $}}
\totalwidth\wd100\advance\totalwidth\wd109
\ifdim\totalwidth>.9\textwidth
	\ifdim\wd100>.45\textwidth
		\box100 ~ \\[-2pt] \hfill \box109
	\else	\box100 \hfill \\[-2pt] ~ \box109\fi
\else \box100 \box109\fi }

 \def \MilTermAbs [l #1 . #2] #3 {{\picolour \setbox102=\hbox{\newb}%
\In {#3} (#1) . \In {#3} (\copy102) . \MilTermRec [#2] {\box102} }}

 \def \MilTermBr[(#1)] #2 { \MilTermRec [#1] #2 }
 \def \MilTermVar[v #1] #2 {{\picolour \Out {#1} <{#2}> }}
 \def \MilTermsub[s #1 #2 := #3] #4 {{\picolour \New {#2} ( \MilTermRec[#1] {#4} \Par \MilSub [{#2} := {#3}] ) }}
 \def \MilTermSub[S #1 #2 := #3] #4 {{\picolour \New {#2} ( \MilTermRec[#1] {#4} \Par \MilSubX [{#2} := {#3}] ) }}

 \def \MilSub [#1 := #2]{\MilSemOne [{#1} := {#2}] }

 \def \MilSubX [#1 := #2]{{\picolour \setbox103=\hbox{\neww}%
\Bang \In {#1} (\copy103) . \MilTerm [#2] {\copy103} }}

 \def \MilSubXPeel [#1 := #2]{{\picolour \setbox103=\hbox{\neww}%
\In {#1} (\copy103) . \MilTermRec [#2] {\copy103} \Par \Bang \In {#1} (\copy103) . \MilTermRec [#2] {\copy103} }}

 \def \MilTermAux[#1] #2 {\piterm {\MilSem [#1] {#2} } }


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 \def \MilSemP[#1]{{\OldSem[#1]\kern-1pt^{\mbox{\scriptsize \textsc p}}}\skp\picolour \resetvariables }

 \def \MilTermP [#1] #2 {\if@om \global \omfalse \MilTermPAux[#1] {#2} \global \omtrue
\resetvariables
\else \MilTermPAux[#1] {#2}\fi}
%
 \def \MilTermPAux [%
 	{\@ifnextchar l{\MilTermPAbs [}%]
	{\@ifnextchar a{\MilTermPApp [}%]
	{\@ifnextchar X{\MilTermPXpp [}%]
	{\@ifnextchar v{\MilTermPVar[}%]
	{\@ifnextchar s{\MilTermPSub[}%]
	{\@ifnextchar ({\MilTermPBr[}%]
		{\MilSemP[\ltermcolour }%]
}}}}}}
%
 \def \MilTermPApp[a #1 #2] #3 {%
\setbox101=\hbox{\newc}%
\setbox104=\hbox{\newz}%
\setbox100=\hbox{{\picolour $\NewA \copy101 (\MilTermPAux [#1] {\copy101} \Par {} $}}%
\global \setbox109=\hbox{{\picolour $\NewA \copy104 ( \Out {\copy101} <\copy104,{#3}> . \MilSubP[{\copy104} := {#2} ] ) ) $}}%
%\global \setbox109=\hbox{{\picolour $\NewA \copy104 ( \Out {\copy101} <{\copy104},{#3}> \Par \Bang { \MilTermP[#2] {\box104} } ) ) $}}%
\totalwidth\wd100\advance\totalwidth\wd109
\ifdim\totalwidth>.9\textwidth
	\ifdim\wd100>.45\textwidth
		\box100 ~ \\[-2pt] \hfill \box109
	\else	\box100 \hfill \\[-2pt] ~ \box109
	\fi
\else \box100 \box109
\fi}
%
 \def \MilTermPAbs [l #1 . #2 ] #3 {{\Red \setbox102=\hbox{\newb}%
\In {#3} (#1,{\copy102}) . \MilTermPAux[#2] {\copy102}
}}
%
 \def \MilTermPBr[<#1>] #2 {{\picolour (\MilTermPAux[{#1}] #2 )}}
 \def \MilTermPVar[v #1] #2 {{\picolour \Out {#1} <#2> }}
 \def \MilTermPSub[s #1 #2 := #3] #4 {{\picolour \New {#2} ( \MilTermP[#1] #4 \Par \MilSubP [#2 := #3] ) }}
 \def \MilsubP [#1 := #2]{\setbox103=\hbox{\neww}
 	{\picolour \Bang \In {#1} (\copy103) . \MilTermPAux [#2] {\copy103} }}
 \def \MilSubP [#1 := #2]{\MilSemPOne [{#1} := {#2}]}
 \def \MilSubPeelP [#1 := #2]{\setbox103=\hbox{\neww}%
	{\picolour \In {#1} (\copy103) . \MilTermPAux [#2] {\copy103} \Par
	\MilSubP [#1 := #2] %\In {#1} (\copy103) . \MilTermPAux [#2] {\copy103} )
	}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 \def \MilSemR[#1]{{\semcolour [\kern-1.75\point[}\kern.6\point \lterm {#1} \kern.6\point{\semcolour ]\kern-1.75\point]^{\kern-1pt\mbox{\scriptsize \textsc r}}
^r}\skp\picolour }

 \def \MilTermR [#1] #2 {\if@om \global \omfalse \MilTermRAux[#1] {#2} \global \omtrue
\resetvariables
\else \MilTermRAux[#1] {#2}\fi}
%
 \def \MilTermRAux [{%]
\@ifnextchar L%
	{\MilTermRAbs [}%]
	{\@ifnextchar A%
		{\MilTermRApp [}%]
	{\@ifnextchar X%
		{\MilTermRXpp [}%]
		{\@ifnextchar V%
			{\MilTermRVar[}%]
			{\@ifnextchar S%
				{\MilTermRSub[}%]
				{\@ifnextchar (%)
					{\MilTermRBr[}%]
					{\MilSemR[\ltermcolour }%]
}}}}}}
%
 \def \MilTermRApp[A #1 #2] #3{%
\setbox101=\hbox{\newc}%
\setbox104=\hbox{\newz}%
\setbox100=\hbox{{\picolour $\NewA \copy101 (\MilTermRAux [#1] {\copy101} \Par {} $}}%
\global \setbox109=\hbox{{\picolour $\NewA \copy104 ( \In {\copy101} (\copy104,{#3}) . \MilSem[\lterm {\copy104 := #2} ]
) ) $}}%
\totalwidth\wd100\advance\totalwidth\wd109
\ifdim\totalwidth>.9\textwidth
	\ifdim\wd100>.45\textwidth
		\box100 ~ \\[-2pt] \hfill \box109
	\else	\box100 \hfill \\[-2pt] ~ \box109
	\fi
\else \box100 \box109
\fi}
%
 \def \MilTermRXpp[X #1 #2] #3{%
\setbox101=\hbox{\newc}%
\setbox104=\hbox{\newz}%
\setbox100=\hbox{{\picolour $\NewA \copy101 (\MilTermRAux [#1] {\copy101} \Par {} $}}%
\global \setbox109=\hbox{{\picolour $ \In {\copy101} (\copy104,y) . \MilsubR [ {\copy104} := {#2} ] \Par \Eq y={#3} ) $}}%
\totalwidth\wd100\advance\totalwidth\wd109
\ifdim\totalwidth>.9\textwidth
	\ifdim\wd100>.45\textwidth
		\box100 ~ \\[-2pt] \hfill \box109
	\else	\box100 \hfill \\[-2pt] ~ \box109
	\fi
\else \box100 \box109
\fi}
%
 \def \MilTermRAbs [L #1 . #2 ] #3 {{\Red \setbox102=\hbox{\newb}%
\New #1{\copy102} ( \MilTermRAux[#2] {\copy102} \Par \Out {#3} <#1,\copy102> ) }}
%
 \def \MilTermRBr[<#1>]{{\picolour (\MilTermRAux[{#1}] )}}
% \def \MilTermRVar[V #1 ] #2 {{\picolour \Out {#2} <{#1}> }}
 \def \MilTermRVar[V #1] #2 {{\picolour \Out {#1} <{#2}> }}
 \def \MilTermRSub[S #1 #2 := #3 ] #4 {{\picolour \New {#2} ( \MilTermR[#1] #4 \Par \MilSub [#2 := #3 ] ) }}
 \def \MilsubR [#1 := #2 ] {{\picolour \setbox103=\hbox{\neww}\Bang ( \In {#1} (\copy103) . \MilTermRAux [#2] {\copy103} ) }}
 \def \MilSubXPeelR [#1 := #2 ] {{\picolour \setbox103=\hbox{\neww}\In {#1} (\copy103) . \MilTermRAux [#2] {\copy103} \Par \Bang ( \In {#1} (\copy103) . \MilTermRAux [#2] {\copy103} ) }}
 \def \MilSubR [#1 := #2 ] {\MilSemOne [{#1} := {#2}]}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def \semPiTwo#1<#2>{\LeftTop{#1}{\ltermcolour #1}\Rightbot\kern-2.5\point\raise5\point\hbox{\semcolour \scriptsize \textsc {#2}}\kern.5\point}
\def \semPiOne#1{\LeftTop{\ltermcolour #1}{#1}\RightBot}
\def \semPi #1{\@ifnextchar<{\semPiTwo{#1}}{\semPiOne{#1}}}

\def \semPiF#1{\@ifnextchar<{\semPiFTwo{#1}}{\semPiFOne{#1}}}
\def \semPiFOne#1{\LeftTop{#1}{#1}\RightBot\kern1pt}
\def \semPiFTwo#1<#2>{\LeftTop{#1}{#1}\Rightbot\kern-2.5\point\raise6\point\hbox{\scriptsize \textsc {\sf #2}}\kern1\point}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 \newcounter{hulpindex}
 \newcounter{indbeta}\setcounter{indbeta}0
 \def \newbeta{\stepcounter{indbeta}{\ifnum\indbeta=1{`b}\else`b_{\theindbeta}\fi}}

 \def \mySem[#1]{{\Sem{{\ltermcolour #1}}}}

 \def \PiLSem[#1] #2 {{\semPi{\LTerm<{#1}>}<s>} \skp {#2} }

 \def \SPiTerm [#1] #2 {\semPi{\LTerm<{#1}>}%<l>
 \piterm {#2} }
 \def \BPiTerm{\Bang \PiTerm}

 \def \PiTerm [#1] #2 {\if@om \resetvariables \global \omfalse {\picolour \PiTermAux[#1] #2 } \global \omtrue \resetvariables \else \PiTermAux[#1] #2\fi}

 \def \PiTermAux[%]
	{\@ifnextchar l{\PiTermAbs[}%]
	{\@ifnextchar a{\PiTermApp[}%]
	{\@ifnextchar d{\PiTermDpp[}%]
	{\@ifnextchar t{\PiTermTpp[}%]
	{\@ifnextchar v{\PiTermVar[}%]
	{\@ifnextchar s{\PiTermsub[}%]
	{\@ifnextchar S{\PiTermSub[}%]
	{\@ifnextchar X{\PiTermXSub[}%]
	{\@ifnextchar({\PiTermBr[}%])
		{\PiLSem[}%]
}}}}}}}}}

 \def \PiTermApp[a #1 #2] #3 {%
\global\setbox103=\hbox{\newc}%
\New \copy103 ( \PiTermAux [#1] {\copy103} \Par 
\In {\copy103} (v,d) . ( \Bang \PiTermAux [#2] v \Par \Eq d={#3} ) ) 
}

 \def \PiTermDpp[d #1 #2] #3 {%
\NewDL \copy105 ( \PiTermAux [#1] e \Par 
	{} \\[-1pt] \tab 
\In e (v,d) . ( \Bang \PiTermAux [#2] v \Par \Eq d={#3} ) ) 
}

 \def \PiTermTpp[t #1 #2] #3 {%
 \setbox105=\hbox{\newc}\setbox106=\hbox{\newb}%
\global\setbox107=\hbox{$\picolour \NewA \copy105 ( \PiTermAux [#1] {\copy105} $}%
\global\setbox108=\hbox{{$ \In {\copy105} (\copy106,d) . (
\New \Out\In {\copy106} (x) . \Bang \PiTermAux [#2] x \Par \Eq d={#3} ) ) $}}%
\totalwidth\wd107\advance\totalwidth\wd108
\ifdim\totalwidth>.85\textwidth
	\ifdim \wd107>.4\textwidth \copy107 \Par {} \quad \\[-1pt] \hfill \copy108
	\else \box107 {} \Par \hfill \\[-1pt] \quad \hfill \box108
	\fi
\else	\box107 \Par \box108
\fi}

 \def \PiTermAbs[l #1 . #2] #3 {%
{\picolour \setbox111=\hbox{\newb}%
\NewA #1\copy111 ( \PiTermAux [#2] \copy111 \Par \Out{#3} <#1,\box111> ) } }

 \def \PiTermVar[v #1] #2 {%
\setbox77=\hbox{$w$}
{\picolour \In {#1} (\copy77) . \Out{#2} <\box77> } }
 
 \def \PiTermsub[s #1 #2 := #3] #4 {%
%\setbox131=\hbox{\newb}
%{\Orange \New {#2\copy131} ( \PiTermAux [#1] {\copy131} \Par \Bang { \PiTermAux [#3] #2 } \Par \Eq{\copy131}={#4} ) }
 \New {#2} ( \PiTermAux [#1] {#4} \Par \Bang { \PiTermAux [#3] #2 } ) }

 \def \PiTermSub[S #1 #2 := #3] #4 {%
 \New {#2} ( \PiTermAux [#1] {#4} \Par \Bang { \PiTermAux [#3] #2 } ) }

 \def \PiTermXSub[X #1 #2 := #3] #4 {%
{\Orange \New {#2} ( \PiTermAux [#1] {#4} \Par \PiTermAux [#3] #2 \Par \Bang { \PiTermAux [\LTerm<#3>] #2 } ) }}

 \def \PiTermBr[<#1>] #2 {{\Orange \PiTermAux [#1] #2 }}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% First Full encoding
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 \def \PiFLSem{\PiLFSem}
 \def \PiLFSem[#1] #2 {{\semPi{\LTerm<{#1}>}<f>} {#2} }
 \def \SPiFTerm[#1] #2 {\PiLFSem[#1] {\picolour #2} }
 \def \BPiLFSem[#1] #2 {\Bang {\semPi{\LTerm<{#1}>}<f>} {#2} }

 \def \BPiFLSem{\Bang \SPiFTerm}
 \def \SPiFLTerm{\SPiFTerm}
 \def \BSPiFLTerm{\Bang \SPiFTerm}
 \def \BPiFTerm{\Bang \PiFTerm}
 \def \BSPiFTerm{\Bang \SPiFTerm}

%
 \def \PiFTerm [#1] #2 {\if@om \omfalse \PiFTermAux[#1] #2 \omtrue \resetvariables \else \PiFTermAux[#1] #2 \fi}

 \def \PiFTermAux[%]
 	{\@ifnextchar l{\PiFTermAbs[}%]
	{\@ifnextchar a{\PiFTermApp[}%]
	{\@ifnextchar u{\PiFTermUnfApp[}%]
	{\@ifnextchar X{\PiFTermXUnfApp[}%]
	{\@ifnextchar d{\PiFTermDlApp[}%]
	{\@ifnextchar e{\PiFTermEDlApp[}%]
	{\@ifnextchar t{\PiFTermTpp[}%]
	{\@ifnextchar v{\PiFTermVar[}%]
	{\@ifnextchar ({\PiFTermBr[}%])
	{\@ifnextchar s{\PiFTermSub[}%]
	{\@ifnextchar Z{\PiFTermDlSub[}%]
	{\@ifnextchar n{\PiFTermName[}%]
	{\@ifnextchar m{\PiFTermMu[}%]
		{\SPiFTerm[}%]
}}}}}}}}}}}}}

 \def \PiFTermApp[a #1 #2] #3 {%\theindb \theindc % LApp
\setbox154=\hbox{$#3$}
\stepcounter{indb}\stepcounter{indc}
\New {\cind}{\bind} ( \PiFTermAux [#1] {\cind} \Par \LSynCell {\bind} [{\cind}] {\box154} \Par \Bang \SPiFTerm [#2] {\bind} )
\addtocounter{indb}{-1}\addtocounter{indc}{-1} % RApp
}

 \def \PiFTermUnfApp[u #1 #2] #3 {% LUpp
\setbox155=\hbox{$#3$} \stepcounter{indb}\stepcounter{indc}
\New {\cind}{\bind} ( \PiFTermAux [#1] {\cind} \Par \LSynCell {\bind} [{\cind}] {\box155} \Par
\PiFTerm [#2] {\bind} {} \Par \Bang \SPiFTerm [#2] {\bind} )
\addtocounter{indb}{-1}\addtocounter{indc}{-1} % RUpp
}

 \def \PiFTermXUnfApp[X #1 #2] #3 {% LUpp
\setbox156=\hbox{$#3$} \stepcounter{indb} \stepcounter{indc}
\New {\cind}{\bind} ( \PiFTermAux [#1] {\cind} \Par \LSynCell {\bind} [{\cind}] {\box156} \Par
\\[-1\point] \dquad
\PiFTerm [#2] {\bind} {} \Par \Bang \SPiFTerm [#2] {\bind} )
\addtocounter{indb}{-1}\addtocounter{indc}{-1} % RUpp
}

 \def \PiFTermDlApp[d #1 #2] #3 {% LDpp
\setbox156=\hbox{$#3$} \stepcounter{indb} \stepcounter{indc}
\New {\cind}{\bind} ( \PiFTermAux [#1] {\cind} \Par
\LSynCell {\bind} [{\cind}] {\box156} \Par  \\[-1pt] ~ \dquad
\Bang \SPiFTerm [#2] {\bind} )
\addtocounter{indb}{-1}\addtocounter{indc}{-1} % RDpp
}

 \def \PiFTermEDlApp[e #1 #2] #3 {% LEpp
\global\setbox157=\hbox{$#3$} \stepcounter{indb}\stepcounter{indc}
\New {\cind}{\bind} ( \PiFTermAux [#1] {\cind} \Par \\[-1pt] \dquad
\LSynCell {\bind} [{\cind}] {\box157} \Par
\Bang \SPiFTerm [#2] {\bind} )
\addtocounter{indb}{-1}\addtocounter{indc}{-1} % REpp
}

\def\relay#1#2{\expandafter\def\csname #1\endcsname{#2}%
}% With this definition, \relay{blah}{bleah} is equivalent to \def\blah{bleah}.

\newsavebox{\Anul}\newsavebox{\Ai}\newsavebox{\Aii}\newsavebox{\Aiii}
\newsavebox{\Aiv}\newsavebox{\Av}\newsavebox{\Avi}\newsavebox{\Avii}

 \def \PiFTermAbs[l #1 . #2] #3 {%\theindb \theindc % LAbs
\global\Adv{\depth}{1} % \the\depth
\ifnum\depth=0\global\sbox{\Anul}{\hbox{$\picolour #3$}}\fi
\ifnum\depth=1\global\sbox{\Ai}{\hbox{$\picolour #3$}}\fi
\ifnum\depth=2\global\sbox{\Aii}{\hbox{$\picolour #3$}}\fi
\ifnum\depth=3\global\sbox{\Aiii}{\hbox{$\picolour #3$}}\fi
\ifnum\depth=4\global\sbox{\Aiv}{\hbox{$\picolour #3$}}\fi
\ifnum\depth=5\global\sbox{\Av}{\hbox{$\picolour #3$}}\fi
\ifnum\depth=6\global\sbox{\Avi}{\hbox{$\picolour #3$}}\fi
\ifnum\depth=7\global\sbox{\Avii}{\hbox{$\picolour #3$}}\fi
%
% \the\depth \theindb
\stepcounter{indb}
\NewA #1{\bind} ( \PiFTermAux [#2] {\bind} \Par
%.\usebox{\Anul}.\usebox{\Aii}.\usebox{\Aiii}.\usebox{\Aiv}.\usebox{\Av}.
%\usebox{\Avi}.\usebox{\Avii}.\usebox{\Aviii}.
\ifnum\depth<-1{A} \else \ifnum\depth<0{B} \else \ifnum\depth<1{C}\fi\fi\fi
\ifnum\depth=0{\Out \usebox{\Ai} <#1,{\bind}> }\fi
\ifnum\depth=1{\Out \usebox{\Ai} <#1,{\bind}> }\fi
\ifnum\depth=2{\Out \usebox{\Aii} <#1,{\bind}> }\fi
\ifnum\depth=3{\Out \usebox{\Aiii} <#1,{\bind}> }\fi
\ifnum\depth=4{\Out \usebox{\Aiv} <#1,{\bind}> }\fi
\ifnum\depth=5{\Out \usebox{\Av} <#1,{\bind}> }\fi
\ifnum\depth=6{\Out \usebox{\Avi} <#1,{\bind}> }\fi
\ifnum\depth=7{\Out \usebox{\Avii} <#1,{\bind}> }\fi
\ifnum\depth=8{\Out \usebox{\Avii} <#1,{\bind}> }\fi
\ifnum\depth>8\Out #3 <#1,b_{\the\depth}>\fi
) \global\Adv{\depth}{-1} \addtocounter{indb}{-1} % RAbs
}

 \def \PiFTermVar[v #1] #2 {\setbox77=\hbox{\neww}
\In {#1} (\copy77) . \Out{#2} <\box77> }

 \def \PiFTermName[n #1 #2] #3 { \PiFTermAux[#2] #1 }

 \def \PiFTermMu[m #1 . #2] #3 { \New #1 ({ \PiFTermAux[#2] {} \Par \BEq #1=#3 }) }

 \def \PiFTermSub[s #1 #2 := #3] #4 {\NewA #2 ( \PiFTermAux [#1] {#4} \Par \Bang \SPiFTerm [{#3}] #2 ) }

 \def \PiFTermDlSub[Z #1 #2 := #3] #4 {\NewA #2 ( \PiFTermAux [#1] {#4} \Par \\ \hfill \Bang \SPiFTerm [{#3}] #2 ) }

\def \PiFTermBr[(#1)] #2 {\PiFTermAux [#1] #2 }


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Head encoding
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 \def \PiLGSem[#1] #2 {{\semPi{\LTerm<{#1}>}<t>} {#2} }
 \def \SPiGTerm[#1] #2 {\PiSemL[#1] {\picolour #2} }
 \def \BPiLGSem[#1] #2 {\Bang {\semPi{\LTerm<{#1}>}<t>} {#2} }

 \def \PiHSem[#1]{\ifnextchar[{\PiHSemwithSub[#1]}{\PiSemGen[{\Bluecol #1}] n }}%]
 \def \PiHSemwithSub[#1][#2]{\setbox129=\hbox{$#1$}
\ifdim\wd129>25\point \PiSemGen[{\Bluecol #1[#2]}] n
\else \PiSemGen[{\Bluecol #1[#2]}] n
\fi}

 \def \BPiHSem{\Bang \PiHSem}

 \def \PiHLSem[#1] #2 {\kern1.5\point {\semPi{\LTerm<{#1}>}<h>} \kern1\point {#2} \kern1\point }
 \def \SPiHLTerm[#1] #2 {\PiHLSem[#1] {\picolour #2} }
 \def \BPiLHSem[#1] #2 {\Bang {\semPi{\LTerm<{#1}>}<h>} {#2} }

 \def \BPiHLSem{\Bang \SPiHLTerm}
 \def \BSPiHLTerm{\Bang \SPiHLTerm}
 \def \BPiHLTerm{\Bang \PiHLTerm}
 \def \BSPiHLTerm{\Bang \SPiHLTerm}

 \def \PiHLTerm [#1] #2 {\if@om \omfalse \PiHLTermAux[#1] #2 \omtrue \resetvariables \else \PiHLTermAux[#1] #2 \fi}

 \def \PiHLTermAux[%]
 	{Aux\@ifnextchar L{\PiHLTermAbs[}%]
	{\@ifnextchar A{\PiHLTermApp[}%]
	{\@ifnextchar D{\PiHLTermDlApp[}%]
	{\@ifnextchar V{\PiHLTermVar[}%]
	{\@ifnextchar ({\PiHLTermBr[}%])
	{\@ifnextchar S{\PiHLTermSub[}%]
	{\@ifnextchar Z{\PiHLTermDlSub[}%]
		{\SPiHLTerm[}%]
}}}}}}}

 \def \PiHLTermAbs[L #1 . #2] #3 {%\theindb \theindc % LAbs
\global\Adv{\depth}{1} % \the\depth
\ifnum\depth=0\global\sbox{\An}{\hbox{$\picolour #3$}}\fi
\ifnum\depth=1\global\sbox{\Ai}{\hbox{$\picolour #3$}}\fi
\ifnum\depth=2\global\sbox{\Aii}{\hbox{$\picolour #3$}}\fi
\ifnum\depth=3\global\sbox{\Aiii}{\hbox{$\picolour #3$}}\fi
\ifnum\depth=4\global\sbox{\Aiv}{\hbox{$\picolour #3$}}\fi
\ifnum\depth=5\global\sbox{\Av}{\hbox{$\picolour #3$}}\fi
\ifnum\depth=6\global\sbox{\Avi}{\hbox{$\picolour #3$}}\fi
\ifnum\depth=7\global\sbox{\Avii}{\hbox{$\picolour #3$}}\fi
%
% \the\depth \theindb
\stepcounter{indb}
\NewA #1{\bind} ( \PiHLTermAux [#2] {\bind} \Par
%.\usebox{\An}.\usebox{\Aii}.\usebox{\Aiii}.\usebox{\Aiv}.\usebox{\Av}.
%\usebox{\Avi}.\usebox{\Avii}.\usebox{\Aviii}.
\ifnum\depth<-1{A} \else \ifnum\depth<0{B} \else \ifnum\depth<1{C}\fi\fi\fi
\ifnum\depth=0{\Out \usebox{\Ai} <#1,{\bind}> }\fi
\ifnum\depth=1{\Out \usebox{\Ai} <#1,{\bind}> }\fi
\ifnum\depth=2{\Out \usebox{\Aii} <#1,{\bind}> }\fi
\ifnum\depth=3{\Out \usebox{\Aiii} <#1,{\bind}> }\fi
\ifnum\depth=4{\Out \usebox{\Aiv} <#1,{\bind}> }\fi
\ifnum\depth=5{\Out \usebox{\Av} <#1,{\bind}> }\fi
\ifnum\depth=6{\Out \usebox{\Avi} <#1,{\bind}> }\fi
\ifnum\depth=7{\Out \usebox{\Avii} <#1,{\bind}> }\fi
\ifnum\depth=8{\Out \usebox{\Avii} <#1,{\bind}> }\fi
\ifnum\depth>8\Out #3 <#1,b_{\the\depth}>\fi
) \global\Adv{\depth}{-1} \addtocounter{indb}{-1} % RAbs
}

 \def \PiHLTermApp[A #1 #2] #3 {%\theindb \theindc % LApp
\setbox154=\hbox{$#3$}
\stepcounter{indc}
\New {\cind} ( \PiHLTermAux [#1] {\cind} \Par \In \cind (v,d) ({ \PiHLTermAux [#2] v \Par {\BEq d=#3 } })
\addtocounter{indc}{-1} % RApp
}

 \def \PiHLTermDlApp[D #1 #2] #3 {%LDpp
\setbox156=\hbox{$#3$} \stepcounter{inde}
\NewDL {\eind} ( \Bang \PiHLTermAux [#1] {\eind} \Par 
	{} \\ \tab 
\In \eind (v,d) ({ \Bang \PiHLTerm [#2] v \Par {\BEq d=#3 } }) )
\addtocounter{indc}{-1} % RDpp
}

\newsavebox{\An}%\newsavebox{\Ai}\newsavebox{\Aii}\newsavebox{\Aiii}
%\newsavebox{\Aiv}\newsavebox{\Av}\newsavebox{\Avi}\newsavebox{\Avii}

  \def \PiHLTermVar[V #1] #2 {\In {#1} (\copy77) . \Out{#2} <\box77> }

 \def \PiHLTermSub[S #1 #2 := #3] #4 {\NewA #2 ( \PiHLTermAux [#1] {#4} \Par \Bang \SPiHLTerm [{#3}] #2 ) }

 \def \PiHLTermDlSub[Z #1 #2 := #3] #4 {\NewA #2 ( \PiHLTermAux [#1] {#4} \Par \\ \hfill \Bang \SPiHLTerm [{#3}] #2 ) }

\def \PiHLTermBr[(#1)] #2 {\PiHLTermAux [#1] #2 }


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Trying a new approach
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 \def \PiRLSem[#1] #2 {{\semPi{\LTerm<#1>}<r>} \skp \piterm {\picolour #2} }

 \def \SPiRLTerm {\PiRLSem} % [#1] #2 {{\semPi{\LTerm<#1>}<r>} \piterm {#2} }

 \def \SPiRTerm{\SPiRLTerm}

 \def \PiRTerm [#1] #2 {\if@om \omfalse \PiRTermAux[#1] #2 \omtrue \resetvariables \else \PiRTermAux[#1] #2 \fi}

 \def \PiRTermAux[{%]
\@ifnextchar L%
	{\PiRTermAbs[}%]
	{\@ifnextchar A%
	{\PiRTermApp[}%]
	{\@ifnextchar T%
	{\PiRTermTpp[}%]
	{\@ifnextchar V%
	{\PiRTermVar[}%]
	{\@ifnextchar S%
	{\PiRTermSub[}%]
	{\@ifnextchar X%
	{\PiRTermXSub[}%]
	{\@ifnextchar(%)
	{\PiRTermBr[}%]
	{\SPiRLTerm[}%]
}}}}}}}
%
 \def \PiRTermApp[A #1 #2] #3 {%
\setbox115=\hbox{\newc}%
\setbox116=\hbox{\newb}%
\global\setbox117=\hbox{$\picolour \NewA \copy115\copy116 ( \PiRTermAux [#1] {\copy115} $}%
\global\setbox118=\hbox{$
\Bang \In {\copy115} (v,d) . ( \Bang \Eq {\copy116}=v \Par \Bang \Eq d={#3} ) \Par \PiRTermAux [#2] {\box116} )
$}%
%\totalwidth\wd117\advance\totalwidth\wd118
%\ifdim\totalwidth>.85\columnwidth
%	\ifdim \wd117>.4\columnwidth \copy117 \Par {} \quad \\[-1pt] \hfill \copy118
%	\else \box117 {} \Par \hfill \\[-1pt] \quad \hfill \box118
%	\fi
%\else
	\box117 \Par \box118
%\fi
}
%
 \def \PiRTermTpp[T #1 #2] #3 {%
\setbox115=\hbox{\newc}%
\setbox116=\hbox{\newb}%
\global\setbox117=\hbox{$\picolour \NewA \copy115\copy116 ( \PiRTermAux [#1] {\copy115} $}%
\global\setbox118=\hbox{$ \Bang \In {\copy115} (v,d) . ( \Bang \Eq {\copy116}=v \Par \Bang \Eq d={#3} ) \Par \PiRTermAux [#2] {\box116} ) $}%
\totalwidth\wd117\advance\totalwidth\wd118
\ifdim\totalwidth>.85\columnwidth
	\ifdim \wd117>.4\columnwidth
		\copy117 \Par {} \quad \\[-1pt] \hfill \copy118
	\else \box117 {} \Par \hfill \\[-1pt] \quad \hfill \box118
	\fi
\else	\box117 \Par \box118
\fi}
%
 \def \PiRTermAbs[L #1 . #2] #3 {{\picolour \setbox111=\hbox{\newb}%
\NewA #1\copy111 ( \PiRTermAux [#2] \copy111 \Par \Bang \Out{#3} <#1,\box111> ) } }
%
 \def \PiRTermVar[V #1] #2 {\setbox77=\hbox{\neww}
\Bang \In {#1} (\copy77) . \Out{#2} <\box77> }
%
 \def \PiRTermSub[S #1 #2 := #3] #4 {\New {#2} ( \PiRTermAux [#1] {#4} \Par \PiRTermAux [#3] #2 ) }
%
 \def \PiRTermXSub[X #1 #2 := #3] #4 {{\Orange \New {#2} ( \PiRTermAux [#1] {#4} \Par \PiRTermAux [#3] #2 \Par \Bang { \PiRTermAux [\LTerm<#3>] #2 } ) }}
%
 \def \PiRTermBr[<#1>] #2 {{\Orange \PiRTermAux [#1] #2 }}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 \def \semPiTermV [#1] #2 {\piterm {{\semPi{#1}<v>}} \piterm {#2} }
 \def \SPiTermV [#1] #2 {\piterm {{\semPi{ \LTerm<#1>}<v>}} \piterm {#2} }

 \def \PiTermV [#1] #2 {\if@om \global \omfalse \PiTermVAux[#1] #2 \global \omtrue \resetvariables
\else \PiTermVAux[#1] #2\fi}

 \def \PiTermVAux[{%]
\@ifnextchar L%
	{\PiTermVAbs[}%]
	{\@ifnextchar A%
	{\PiTermVApp[}%]
	{\@ifnextchar O%
	{\PiTermVOpp[}%]
	{\@ifnextchar V%
	{\PiTermVVar[}%]
	{\@ifnextchar S%
	{\PiTermVSub[}%]
	{\@ifnextchar X%
	{\PiTermVXSub[}%]
	{\@ifnextchar(%)
	{\PiTermVBr[}%]
	{\@ifnextchar I%
	{\PiTermVId[}%]
	{\SPiTermV[}%]
}}}}}}}}
%
 \def \PiTermVApp[A #1 #2] #3 {%
\setbox102=\hbox{\newv}%
\setbox103=\hbox{\newz}%
\setbox104=\hbox{\newy}%
\setbox105=\hbox{\newc}%
\setbox106=\hbox{\newb}%
\setbox107=\hbox{$\picolour \NewA \copy105\copy106 ( \PiTermVAux [#1] {\copy105} $}%
\global\setbox108=\hbox{$
%	\New {\copy106} ({
		\In {\copy105}
			(\copy103,\copy104) .
				( \Eq {\copy106}={\copy103} \Par \Eq {\copy104}={#3} )
		\Par \Bang { \PiTermVAux [#2] {\copy106} }
%	})
 ) $}%
\totalwidth\wd107\advance\totalwidth\wd108
\ifdim\totalwidth>.85\textwidth
	\ifdim \wd107>.\wd108 \box107 \Par {} \quad \\[-1pt] \hfill \box108
	\else \box107 \Par {} \hfill \\[-1pt] \quad \hfill \box108
	\fi
\else	\box107 \Par \box108
\fi}
%
 \def \PiTermVOpp[O #1 #2] #3 {%
\setbox102=\hbox{\newv}%
\setbox103=\hbox{\newz}%
\setbox104=\hbox{\newy}%
\setbox105=\hbox{\newc}%
\setbox106=\hbox{\newb}%
\setbox107=\hbox{$\picolour \NewA \copy105\copy106) ( \PiTermVAux [#1] {\copy105} $}%
\global\setbox108=\hbox{$
%	\New {\copy106}
%		({
		\In {\copy105}
			(\copy103,\copy104) .
				( \Eq {\copy106}={\copy103} \Par \Eq {\copy104}={#3} )
		\Par \PiTermVAux [#2] {\copy106}
		\Par \Bang { \SPiTermV [#2] {\copy106} }
%	})
 ) $}%
\totalwidth\wd107\advance\totalwidth\wd108
\ifdim\totalwidth>.85\textwidth
	\ifdim \wd107>\wd108 \box107 \Par {} \quad \\[-1pt] \hfill \box108
	\else \box107 \Par {} \\[-1pt] \quad \hfill \box108
	\fi
\else	\box107 \Par \box108
\fi}
%
 \def \PiTermVAbs[L #1 . #2] #3 {%
\setbox111=\hbox{\newb}%
\setbox112=\hbox{\newv}%
 {\picol
% \New {\copy112} \Out {#3} <\copy112> .
\New {#1\copy111} ( \Out{#3} <#1,\copy111> \Par \PiTermVAux [#2] {\box111} )
}}
%
 \def \PiTermVVar[V #1] #2 {{\picolour \In {#1} (w) . \Out{#2} <w> } }
%
 \def \PiTermVSub[S #1 <#2 := #3>] #4 {\setbox131=\hbox{\newb}
{\Orange \New {#2\copy131} ( \PiTermVAux [#1] {\copy131} \Par \Bang { \PiTermVAux [#3] #2 } \Par \Eq{\copy131}={#4} ) }}
%
 \def \PiTermVSub[S #1 <#2 := #3>] #4 {\New {#2} ( \PiTermVAux [#1] {#4} \Par \Bang { \PiTermVAux [#3] #2 } ) }
%
 \def \PiTermVXSub[X #1 <#2 := #3>] #4 {{\Orange \New {#2} ( \PiTermVAux [#1] {#4} \Par \PiTermVAux [#3] #2 \Par \Bang { \PiTermVAux [\LTerm<#3>] #2 } ) }}
%
 \def \PiTermVBr[<#1>] #2 {{\Orange \PiTermVAux [#1] #2 }}
 \def \PiTermVId[I #1] #2 {\semPiTermV[#1] #2 }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \def \SPiTermAlt [#1] #2 {\piterm {\semPi{ \LTerm<#1>}<i> } \piterm {#2} }

 \def \PiTermAlt [#1] #2 {\if@om \global \omfalse \PiTermAltAux[#1] #2 \global \omtrue
\resetvariables
\else \PiTermAltAux[#1] #2\fi }
 \def \PiTermAltAux[{%]
\@ifnextchar L%
	{\PiTermAltAbs[}%]
	{\@ifnextchar A%
		{\PiTermAltApp[}%]
		{\@ifnextchar X%
			{\PiTermAltXpp[}%]
			{\@ifnextchar V%
				{\PiTermAltVar[}%]
				{\@ifnextchar S%
					{\PiTermAltSub[}%]
					{\@ifnextchar T%
						{\PiTermAltMultiSub[}%]
						{\@ifnextchar(%)
							{\PiTermAltBr[}%]
							{\SPiTermAlt[}%]
} } } } } } }
%
 \def \PiTermAltApp[A #1 #2] #3 {%
\setbox104=\hbox{\neww}%
\setbox105=\hbox{\newc}%
\setbox106=\hbox{\newb}%
\global\setbox107=\hbox{$\picolour \NewA \copy105 ( \PiTermAltAux[#1] {\copy105} $}%
\global\setbox108=\hbox{$ \In {\copy105} (\copy106,d) .
({ \Bang { \In {\box106} (\copy104) . \PiTermAltAux [#2] {\box104} } \Par \Eq d={#3}
}) )$}%
\totalwidth\wd107\advance\totalwidth\wd108
\ifdim\totalwidth>.85\textwidth
	\ifdim \wd107>.4\textwidth \copy107 \Par {} \quad \\[-1pt] \hfill \copy108
	\else \box107 \Par {} \hfill \\[-1pt] \quad \hfill \box108
	\fi
\else	\box107 \Par \box108
\fi}
%
 \def \PiTermAltAbs[L #1 . #2] #3 {{\picolour \setbox111=\hbox{\newd}%
\NewA #1\copy111 ( \PiTermAltAux [#2] {\copy111} \Par \Out{#3} <#1,\box111> ) } }
%
 \def \PiTermAltVar[V #1] #2 {{\picolour \setbox116=\hbox{\newz}%
\New {\copy116} ({ \Out {#1} <\copy116> \Par \In {\box116} (w) . \Out {#2} <w> }) }}
%
% \def \PiTermAltSub[S #1 <#2 := #3>] #4 {\setbox131=\hbox{\newb}
%{\Orange \New {#2\copy131} ( \PiTermAlt[#1] {\copy131} \Par \Bang { \PiTermAlt[#3] #2 } \Par \Eq{\copy131}={#4} ) }}
%
 \def \PiTermAltSub[S #1 <#2 := #3>] #4 {\setbox116=\hbox{\neww}%
\New {#2} ( \PiTermAltAux[#1] {#4} \Par \Bang { \In {#2} (\copy116) . \PiTermAltAux[#3] {\box116} } ) }
%
 \def \PiTermAltMultiSub[T #1 <#2 := #3>] #4 {{\Orange \New {\Vec{#2}} ( \PiTermAltAux[#1] {#4} \Par \Vec{ \Bang { \PiTermAltAux[#3] #2 } \, } ) }}
%
 \def \PiTermAltBr[<#1>] #2 {{\Orange \PiTermAltAux [#1] #2 }}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 \def \EqOpt#1=#2 {\Out {#1} <#1>}
 \def \EqOpt#1=#2 {{#1} {=} {#2}}%{\In {#1} . \Out {#2} }

 \def \SPiTermOpt[#1] #2 {{\semPi{\LTerm<{#1}>}<t>}\piterm{#2} }
 \def \SPiTermopt[#1]{\semPi{\LTerm<#1>}<o>}

 \def \PiTermOpt[#1] #2 {\if@om \global \omfalse \PiTermOptAux[#1] #2 \global \omtrue \resetvariables \else \PiTermOptAux[#1] #2 \fi}

 \def \PiTermOptAux[%]
	{\@ifnextchar a{\PiTermOptApp[}%]
	{\@ifnextchar d{\PiTermOptDpp[}%]
	{\@ifnextchar X{\PiTermOptXpp[}%]
 	{\@ifnextchar l{\PiTermOptAbs[}%]
	{\@ifnextchar v{\PiTermOptVar[}%]
	{\@ifnextchar s{\PiTermOptsub[}%]
	{\@ifnextchar S{\PiTermOptSub[}%]
	{\@ifnextchar t{\PiTermOptMultiSub[}%]
	{\@ifnextchar c{\PiTermOptCont[}%]
	{\@ifnextchar({\PiTermOptBr[}%])
		{\SPiTermOpt[}%]
}}}}}}}}}}
%
\newdimen \totalwidth

 \def \PiTermOptApp[a #1 #2] #3 {\setbox104=\hbox{\neww}\setbox105=\hbox{\newc}\setbox106=\hbox{\newv}\setbox111=\hbox{\newd}%
\global\setbox107=\hbox{$\picolour \NewA \copy105 ( \PiTermOptAux[#1] {\copy105} $}%
\global\setbox108=\hbox{$ \In {\copy105} (v,d) . ( \SPiTermOptXsub [v := {\LTerm<{#2}>}] \Par \Eq d={#3} ) ) $}%
\totalwidth\wd107\advance\totalwidth\wd108
\ifdim\totalwidth>.85\textwidth
	\ifdim \wd107>.4\textwidth \copy107 \Par {} \quad \\[-1pt] \hfill \copy108
	\else \box107 \Par {} \hfill \\[-1pt] \quad \hfill \box108
	\fi
\else	\box107 \Par \box108
\fi}

 \def \PiTermOptDpp[d #1 #2] #3 {\setbox104=\hbox{\neww}\global\setbox105=\hbox{\newc}\setbox106=\hbox{\newv}\setbox111=\hbox{\newd}%
\NewA \copy105 ( \PiTermOptAux[#1] {\copy105} 
\Par \quad {} \hfill \\[-1pt] \quad \hfill 
\In {\copy105} (v,d) . ( \SPiTermOptXsub [v := {\LTerm<{#2}>}] \Par \Eq d={#3} ) ) }

 \def \PiTermOptXpp[X #1 #2] #3 {\setbox104=\hbox{\neww}\setbox105=\hbox{\newc}\setbox106=\hbox{\newb}\setbox111=\hbox{\newd}%
\global\setbox107=\hbox{$\picolour \NewA \copy105 ( \PiTermOptAux[#1] {\copy105} $}%
\global\setbox108=\hbox{$ \In {\copy105} (\copy106,\copy111) .
( \PiTermOptXsub [{\copy106} := {#2}] \Par \Eq {\box111}={#3} ) ) $}%
\totalwidth\wd107\advance\totalwidth\wd108
\ifdim\totalwidth>.85\textwidth
	\ifdim \wd107>.4\textwidth \copy107 \Par {} \quad \\[-1pt] \hfill \copy108
	\else \box107 \Par {} \hfill \\[-1pt] \quad \hfill \box108
	\fi
\else	\box107 \Par \box108
\fi}

 \def \PiTermOptAbs[l #1 . #2] #3 {\global\setbox111=\hbox{\newb}%
\NewA #1\copy111 ( \PiTermOptAux [#2] {\copy111} \Par \Out{#3} <#1,\box111> ) }

 \def \PiTermOptAbs[l #1 . #2] #3 {%\theindb \theindc % LAbs
\global\Adv{\depth}{1} % \the\depth
\ifnum\depth=0\global\sbox{\Anul}{\hbox{$\picolour #3$}}\fi
\ifnum\depth=1\global\sbox{\Ai}{\hbox{$\picolour #3$}}\fi
\ifnum\depth=2\global\sbox{\Aii}{\hbox{$\picolour #3$}}\fi
\ifnum\depth=3\global\sbox{\Aiii}{\hbox{$\picolour #3$}}\fi
\ifnum\depth=4\global\sbox{\Aiv}{\hbox{$\picolour #3$}}\fi
\ifnum\depth=5\global\sbox{\Av}{\hbox{$\picolour #3$}}\fi
\ifnum\depth=6\global\sbox{\Avi}{\hbox{$\picolour #3$}}\fi
\ifnum\depth=7\global\sbox{\Avii}{\hbox{$\picolour #3$}}\fi
%
% \the\depth \theindb
\stepcounter{indb}
\NewA #1{\bind} ( \PiTermOptAux [#2] {\bind} \Par
%.\usebox{\Anul}.\usebox{\Aii}.\usebox{\Aiii}.\usebox{\Aiv}.\usebox{\Av}.
%\usebox{\Avi}.\usebox{\Avii}.\usebox{\Aviii}.
\ifnum\depth<-1{A} \else \ifnum\depth<0{B} \else \ifnum\depth<1{C}\fi\fi\fi
\ifnum\depth=0{\Out \usebox{\Ai} <#1,{\bind}> }\fi
\ifnum\depth=1{\Out \usebox{\Ai} <#1,{\bind}> }\fi
\ifnum\depth=2{\Out \usebox{\Aii} <#1,{\bind}> }\fi
\ifnum\depth=3{\Out \usebox{\Aiii} <#1,{\bind}> }\fi
\ifnum\depth=4{\Out \usebox{\Aiv} <#1,{\bind}> }\fi
\ifnum\depth=5{\Out \usebox{\Av} <#1,{\bind}> }\fi
\ifnum\depth=6{\Out \usebox{\Avi} <#1,{\bind}> }\fi
\ifnum\depth=7{\Out \usebox{\Avii} <#1,{\bind}> }\fi
\ifnum\depth=8{\Out \usebox{\Avii} <#1,{\bind}> }\fi
\ifnum\depth>8\Out #3 <#1,b_{\the\depth}>\fi
) \global\Adv{\depth}{-1} \addtocounter{indb}{-1} % RAbs
}

 \def \PiTermOptVar[v #1] #2 {\setbox141=\hbox{\newz}%
{\picolour \In {#1} (\copy141) . \In {\box141} (u) . \Out {#2} <u> }}

 \def \PiTermOptsub[s #1 #2 := #3] #4 {%
\New {#2} ( \PiTermOptAux[#1] {#4} \Par \SPiTermOptXsub [{#2} := {#3}] )}

% \def \PiTermOptSub[S #1 #2 := #3] {%\setbox131=\hbox{\neww}
%\Bang { \New w ({ \Out {#1} <w> . \PiTermOptAux[#2] w }) }}

 \def \PiTermOptSub[S #1 #2 := #3] #4 {%
\New {#2} ( \PiTermOptAux[#1] {#4} \Par \PiTermOptXsub [{#2} := {#3}] )}

 \def \PiTermOptMultiSub[t #1 #2 := #3 ] #4 {{\Orange \New {\Vec{#2}} ( \PiTermOptAux[#1] {#4} \Par \Vec{ \Bang { \PiTermOptAux[#3] #2 } \, } ) }}

 \def \PiTermOptCont[c #1 := #2 . #3] #4 {\In #1 (v,d) . ( \PiExSub v := {#2} \Par \Eq d=#3 ) }

 \def \PiTermOptBr[(#1)] #2 {{\Orange \PiTermOptAux [#1] #2 }}

 \def \PiTermOptXsub [#1 := #2]{\New w ( \Bang \Out {#1} <w> . \PiTermOptAux [#2] w )}

 \def \SPiTermOptXsub [#1 := #2]{\semPi{\lambdaterm {#1}:={#2} }}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 \def \SPiTermB[#1] #2 {{\Sem{ \LTerm<#1>}'} \skp \piterm {#2} }
 \def \PiSemB[#1] #2 {{\Sem{#1}}' \skp #2 }
 \def \PiTermB [#1] #2 {%
 	\if@om \global \omfalse \PiTermBAux[#1] #2 \global \omtrue \resetvariables
	\else \PiTermBAux[#1] #2
	\fi}
%
 \def \PiTermBAux [%
 	{\@ifnextchar l{\PiTermBAbs[}%]
	{\@ifnextchar a{\PiTermBApp[}%]
	{\@ifnextchar v{\PiTermBVar[}%]
	{\@ifnextchar s{\PiTermBSub[}%]
	{\@ifnextchar ({\PiTermBBr[}%]
		{\SPiTermB[}%]
}}}}}
%
\newdimen\totalwidth
%
 \def \PiTermBApp[a #1 #2] #3 {\setbox105=\hbox{\newc}\setbox106=\hbox{\newb}%
\setbox107=\hbox{{\Orange $\NewA \copy105 {\Green (} \PiTermBAux[#1] {\copy105} $}}%
\global\setbox108=\hbox{{\Orange $ \In {\copy105} (\copy106) . \In {\copy105} (d) . ( \Bang \PiTermBAux [#2] {\copy106} \Par \Bang { \Eq d={#3} } ) {\Green )} $}}%
\totalwidth\wd107\advance\totalwidth\wd108
\ifdim\totalwidth>.8\textwidth
	\ifdim\wd107>.4\textwidth \box107 \Par {} \quad \\[-1pt] \hfill \box108
	\else \box107 {} \Par \hfill \\[-1pt] \quad \hfill \box108
	\fi
\else	\box107 \Par \box108
\fi}

 \def \PiTermBApp[a #1 #2] #3 {%
\setbox104=\hbox{\neww}%
\setbox105=\hbox{\newc}%
\setbox106=\hbox{\newb}%
\setbox111=\hbox{\newd}%
\global\setbox107=\hbox{$\picolour \NewA \copy105 ( \PiTermBAux[#1] {\copy105} $}%
\global\setbox108=\hbox{$ \In {\copy105} (\copy106) . \In {\copy105} (\copy111) .
({ \Bang { \New {\copy104} ({ \Out {\box106} <\copy104> . \PiTermBAux [#2] {\box104} })
} \Par \Bang \Eq {\box111}={#3} }) ) $}%
\totalwidth\wd107\advance\totalwidth\wd108
\ifdim\totalwidth>.85\textwidth
	\ifdim \wd107>.4\textwidth \copy107 \Par {} \quad \\[-1pt] \hfill \copy108
	\else \box107 \Par {} \hfill \\[-1pt] \quad \hfill \box108
	\fi
\else	\box107 \Par \box108
\fi}
%
 \def \PiTermBAbs[l #1 . #2] #3 {{\Orange \setbox111=\hbox{\newb}\NewA #1\copy111 ( \PiTermBAux [#2] {\copy111} \Par \Out{#3} <#1> \Par \Out{#3} <\box111> ) }}
% \def \PiTermBSub[S #1 #2 := #3] #4 {{\Orange \New {#2} ( \PiTermB[#1] #4 \Par \Bang { \PiTermB[#3] #2 } ) }}
 \def \PiTermBSub[S <#1 := #2>] {\setbox131=\hbox{\neww}
\Bang { \New {\copy131} ({ \Out {#1} <\copy131> . \PiTermB[#2] {\box131} }) }
}
%
 \def \PiTermBBr[<#1>]{\Orange \PiTermBAux[#1] }
%
 \def \PiTermBVar[v #1] #2 {%\Bang
 \Orange \In {#1} (w) . \Out{#2} <w> }

 \def \PiTermBVar[v #1] #2 {\setbox141=\hbox{\newz}\setbox142=\hbox{\neww}%
{\picolour \In {#1} (\copy141) . \Bang \In {\box141} (\copy142) . \Out {#2} <\box142> }}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def \SanH (#1) <#2> {{\cal H} \, \Sem{#1} \, \langle#2\rangle}

 \def \SanSemAux#1{%
{\semcolour %{\cal U}
[\kern-1.75\point[}\kern.6\point \lterm {#1} \kern.6\point{\semcolour ]\kern-1.75\point]
^{\mbox{\scriptsize \textsc u}}}\picolour \resetvariables}

 \def \SSanTerm [#1]{\SanSem[\LTerm<#1>]}

 \def \SanSem[#1] #2 {\setbox66=\hbox{${#2}$}%
\ifdim \wd66<1pt {\SanSemAux{#1}} \else \SanSemAux{#1} \box66 \picolour \fi}

 \def \SanTerm [#1] #2 {\if@om \global \omfalse \SanTermAux[#1] #2 \global \omtrue \resetvariables \else \SanTermAux[#1] #2\fi}

 \def \SanTermAux [%
 	{\@ifnextchar l{\SanTermAbs[}%]
	{\@ifnextchar a{\SanTermApp[}%]
	{\@ifnextchar X{\SanTermXpp[}%]
	{\@ifnextchar d{\SanTermDub[}%]
	{\@ifnextchar v{\SanTermVar[}%]
	{\@ifnextchar s{\SanTermsub[}%]
	{\@ifnextchar S{\SanTermSub[}%]
	{\@ifnextchar ({\SanTermBr[}%]
	{\@ifnextchar <{\SanTermEntry[}%]
		{\SanSem [}%]
}}}}}}}}}

 \def \SanTermXpp [X #1 #2] #3 {\setbox177=\hbox{\newq}\setbox178=\hbox{\newv}\setbox179=\hbox{\newx}\setbox180=\hbox{\neww}%
\setbox181=\hbox{$ \NewA \copy177 ( \SanTermAux [#1] {\copy177} $}%
\global\setbox182=\hbox{$ \In {\copy177} (\copy178) . \New {\copy179} ({ \Out {\box178} <\copy179,#3> . \Bang { \In {\box179} (\copy180) . \SanTermAux [#2] {\box180} } }) ) $}%
\box181 \Par \box182
}

 \def \SanTermApp [a #1 #2] #3 {\setbox177=\hbox{\newq}\setbox178=\hbox{\newv}\setbox179=\hbox{\newx}\setbox180=\hbox{\neww}%
\setbox181=\hbox{$ \NewA \copy177 ( \SanTermAux [#1] {\copy177} $}%
\global\setbox182=\hbox{$ \In {\copy177} (\copy178) . \New {\copy179} ({ \Out {\box178} <\copy179,#3> . \SanTermEntry[<\box179 := #2>] }) ) $}
\box181 \Par \box182
}

 \def \SanTermAbs[l #1 . #2] #3 {\setbox172=\hbox{\newv}\setbox173=\hbox{\newq}%
	\New {\copy172} ( \Out {#3} <{\copy172}> .
		\Bang { \In {\box172} (#1,\copy173) . \SanTermAux [#2] {\box173} } )%
}

 \def \SanTermsub[s #1 #2 := #3] #4 {\global \setbox171=\hbox{\neww}%
\New {#2} ({ \SanTermAux [#1] {#4} \Par \SanTermEntry[<{#2} := {#3}>] })
}
 \def \SanTermSub[S #1 #2 := #3] #4 {\global \setbox171=\hbox{\neww}%
\New {#2} ({ \SanTermAux [#1] {#4} \Par \SanSubX [#2 := #3] })
}

 \def \SanTermDub[d #1 #2 := #3] #4 {\global \setbox171=\hbox{\neww}%
\NewA #2 ( \SanTermAux [#1] {#4} \Par {} \\ \hfill \Bang { \In {#2} (\copy171) . \SanTermAux [#3] {\box171} } )
}

%\SanRhs q v x w p [M_n]
 \def \SanRhs #1 #2 #3 #4 #5 [#6] {%
\In {#1} (#2) . \New {#3} ({ \Out {#2} <#3,#5> . \SanTermEntry[<{#3} := {#6}>] }) )}

 \def \Sansub [#1 := #2]{\setbox177=\hbox{\newq}\setbox178=\hbox{\newv}\setbox179=\hbox{\newx}\setbox180=\hbox{\neww}%
			\Bang { \In {\box179} (\copy180) . \SanTermAux [#2] {\box180} }
}

 \def \SanTermBr[<#1>]{\Orange \SanTermAux[#1] }
 \def \SanTermVar[v #1] #2 {\Out{#1} <#2> }
 \def \SanTermEntry [<#1 := #2>]{\SanSem[{ {#1} := {#2} }] }%
 \def \SanSub[#1 := #2]{\SanSem[#1 := #2] {} }
 \def \SanSubX[#1 := #2]{\Bang \In #1 (w) . \SanSem[#2] w }

% \def \SanTermVar[V #1] #2 {\setbox180=\hbox{\neww}\Orange \In{#1} (\copy180) . \Out {\box180} <#2> }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 \def \SanCBVSemAux#1{%
{\semcolour {\cal U}[\kern-1.75\point[}\kern.6\point \lterm {#1} \kern.6\point{\semcolour ]\kern-1.75\point]^v}}

 \def \SSanCBVTerm [#1]{\SanCBVSem[\LTerm<#1>]}

 \def \SanCBVSem[#1] #2 {\setbox66=\hbox{${#2}$}%
\ifdim \wd66<1pt {\SanCBVSemAux{#1}}%
\else \SanCBVSemAux{#1}\, \box66 \picolour %
\fi}
 \def \SanCBVTerm [#1] #2 {\if@om \global \omfalse \SanCBVTermAux[#1] #2 \global \omtrue \resetvariables
\else \SanCBVTermAux[#1] #2\fi}
%
 \def \SanCBVTermAux [{%]
\@ifnextchar L%
	{\SanCBVTermAbs[}%]
	{\@ifnextchar A%
		{\SanCBVTermApp[}%]
		{\@ifnextchar D%
			{\SanCBVTermDub[}%]
			{\@ifnextchar V%
				{\SanCBVTermVar[}%]
				{\@ifnextchar S%
					{\SanCBVTermSub[}%]
					{\@ifnextchar (%
						{\SanCBVTermBr[}%]
						{\SanCBVSem [}%]
}}}}}}
%
 \def \SanCBVTermApp [A #1 #2] #3 {%
\global \setbox176=\hbox{\newr}%
\setbox175=\hbox{\newr}%
\setbox177=\hbox{\newq}%
\setbox178=\hbox{\newv}%
\setbox179=\hbox{\newx}%
\setbox180=\hbox{\neww}%
\setbox181=\hbox{$ \NewA \copy177 ( \SanCBVTermAux [#1] {\copy177} \Par \In {\copy177} (\copy178) . 	\NewA \copy176
 $}%
\global\setbox182=\hbox{$
({ \SanCBVTermAux [#2] {\copy176} \Par
		\In {\box176} (\copy180) . \New \copy179 \Out \box178 <\copy179,#3> .
			\Bang { \In {\box179} (\copy175) . \Out{\box175} <\box180> }
	})
) $}%
\totalwidth\wd181\advance\totalwidth\wd182
\ifdim\totalwidth>.85\textwidth
	\ifdim \wd181>.4\textwidth \copy181 \quad \\[-1pt] \hfill \copy182
	\else \box181 \hfill \\[-1pt] \quad \hfill \box182
	\fi
\else	\box181 \box182
\fi
%\box181 \Par \box182
}
%
 \def \SanCBVTermAbs[L #1 . #2] #3 {%
\setbox172=\hbox{\newv}%
\setbox173=\hbox{\newq}%
	\New {\copy172} ( \Out {#3} <{\copy172}> .
		\Bang { \In {\box172} (#1,\copy173) . \SanCBVTermAux [#2] {\box173} } )%
}
%
 \def \SanCBVTermSub[S #1 <#2 := #3>] #4 {%
\global \setbox171=\hbox{\neww}%
\New {#2} ({ \SanCBVTermAux [#1] {#4} \Par
		\Bang { \In {#2} (\copy171) . \SanCBVTermAux [#3] {\box171} } })
}
 \def \SanCBVTermDub[DL #1 <#2 := #3>] #4 {%
\global \setbox171=\hbox{\neww}%
\NewA #2 ( \SanCBVTermAux [#1] {#4} \Par
{} \\ \hfill
		\Bang { \In {#2} (\copy171) . \SanCBVTermAux [#3] {\box171} } )
}
%
%\SanCBVRhs q v x w p [M_n]
 \def \SanCBVRhs #1 #2 #3 #4 #5 [#6] {%
\In {#1} <#2> .
	\New {#3} ({
		\Out {#2} <#3,#5> .
			\Bang { \In {#3} (#4) . \SanCBVTermAux [#6] {#4} }
	})
)}
%
 \def \SanCBVsub [#1 := #2]{%
\setbox177=\hbox{\newq}%
\setbox178=\hbox{\newv}%
\setbox179=\hbox{\newx}%
\setbox180=\hbox{\neww}%
\global\setbox182=\hbox{$
	\New {\copy179} ({
		\Out {\box178} <\copy179,#1> .
			\Bang { \In {\box179} (\copy180) . \SanCBVTermAux [#2] {\box180} }
	})
) $}%
}
%
 \def \SanCBVTermBr[<#1>]{\Orange \SanCBVTermAux[#1] }
%
 \def \SanCBVTermVar[V #1] #2 {\Out{#1} <#2> }
% \def \SanTermVar[V #1] #2 {\setbox180=\hbox{\neww}\Orange \In{#1} (\copy180) . \Out {\box180} <#2> }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newrgbcolor{lightredcol}{1 0.05 0.05}
\newrgbcolor{Redcol}{0.75 0.05 0.05}
\newrgbcolor{Greencol}{0 0.5 0}
\newrgbcolor{Bluecol}{0.05 0.05 0.75}


 \def \rightharpoonupfill@#1{\setboxz@h{$#1-\m@th$}\ht\z@\z@
 $#1\m@th\copy\z@\mkern-6mu\cleaders
 \hbox{$#1\mkern-2mu\box\z@\mkern-2mu$}\hfill
 \mkern-6mu\mathord\rightharpoonup$}

 \def \overrightharpoonup{\mathpalette\overrightharpoonup@}
 \def \overrightharpoonup@#1#2{\vbox{\ialign{##\crcr\rightharpoonupfill@#1\crcr
 \noalign{\kern-\ex@\nointerlineskip}$\m@th\hfil#1#2\hfil$\crcr}}}

 \def \stat#1#2{\mbox{${\picolour #1}{:}{\typecolour #2}$}}

 \def \PairIn{\textsl{pair-in}}
 \def \PairOut{\textsl{pair-out}}
 \def \OutRule{\textsl{out}}
 \def \InRule{\textsl{in}}
 \def \head <#1> {\textsl{h}\,<#1> }

 \def \free{\textsl{free}}
 \def \Trans{\@ifnextchar({\TransBr}{\textsl{T}}}%)
 \def \TransBr<#1>{\textsl{T}\skp<#1>}
 \def \Dom<#1>{\textsl{Dom}\skp<#1>}
 \def \Domc<#1>{\textsl{Dom}_c\skp<#1>}

 \def \Bt{\@ifnextchar_{\BtUn}{\BtAux}}
 \def \BtAux{\@ifnextchar({\BtBr}{\textsl{BT}}}%)
 \def \BtUn_#1{\@ifnextchar({\BtUnBr_{#1}}{\textsl{BT}_{#1}}}%)
 \def \BtUnBr_#1<#2>{\textsl{BT}_{#1}\skp<#2>}
 \def \BtBr<#1>{\textsl{BT}\skp<#1>}

 \def \BT{\textsf{B}}

 \def \K{\@ifnextchar_{\Kunder}{\textsl{K}\kern1pt}}
 \def \Kunder_#1{\textsl{K}\kern1pt_{#1}}

 \def \cc{\textsf{cc}}

%\def \PiTrTwo[#1]#2{\PiSem[{\ltermcolour #1}] \, {\termcolour #2}}
\def \PiTranV[#1]#2{\PiSem[{\ltermcolour #1}] \, {\termcolour #2}}
\def \PiTranC#1[#2]{{\termcolour #1} \, \PiSem[{\ltermcolour #2}]\,}
\def \PiTranAux[#1]{\@ifnextchar\bgroup{\PiTranV[{#1}]}{\PiSem[{\ltermcolour #1}] \, }}
\def \PiTran{\@ifnextchar[{\PiTranAux}{\PiTranC}}%]

\def \PiSubRtwo #1 / #2 { \Bang \New `g ( \Out #2 <`g> . #1 ) }
\def \PiSubRthree #1 #2 / #3 { \Bang \New #2 ( \Out #3 <`g> . #1{#2} ) }
\def \PiSubR #1 {\@ifnextchar/{}{}}

\def \PiSubR #1 #2 / #3 { \Bang \New #2 ( \Out #3 <#2> . #1{#2} ) }


\def \BPiTranTerm[#1]#2{\Bang \PiTran[#1]{#2}}
\def \BPiTranCont#1[#2]{\Bang \PiTran{#1}[#2]}
\def \BPiTran{\@ifnextchar[{\BPiTranTerm}{\BPiTranCont}}%]

%\def \PiRTrOne[#1]{\PiSem[{\ltermcolour #1}]<r> }
%\def \PiRTrTwo[#1]#2{\PiRTrOne[{#1}] \, {\termcolour #2}}
%\def \PiRTran[#1]{\@ifnextchar{\bgroup}{\PiRTrTwo[{#1}]}{\PiRTrOne[{#1}] }}

\def \PiRTrOne[#1]{ \PiSem[\picolour {\ltermcolour #1}]<r> }
\def \PiRTrTwo[#1]#2{ \PiRTrOne[{#1}] \, {\termcolour #2} }
\def \PiRTranV[#1]#2{ \PiRTrOne[{#1}] \, {\termcolour #2} }
\def \PiRTranC#1[#2]{ {\termcolour #1} \, \PiRTrOne[{#2}] }
\def \PiRTranAux[#1]{ \@ifnextchar\bgroup{\PiRTrTwo[{#1}]}{\PiRTrOne[{#1}] }}
\def \PiRTran{\@ifnextchar[{\PiRTranAux}{\PiRTranC}}%]

\def \BPiRTranTerm[#1]#2{\Bang \PiTran[{\ltermcolour #1}]{#2}}
\def \BPiRTranCont#1[#2]{\Bang \PiTran{#1}[#2]}
\def \BPiRTran{\@ifnextchar[{\BPiRTranTerm}{\BPiRTranCont}}%]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Lmu encoding
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \def \PiLMuSem[#1] #2 {{\semPi{\LTerm<{#1}>}} {#2} }

 \def \PiLmuSem[#1]{\ifnextchar[{\PiLmuSemwithSub[#1]}{{\semPi{\LTerm<{#1}>}}}} %]
 \def \PiLmuSemwithSub[#1][#2]{\setbox129=\hbox{$#1$}
\ifdim\wd129>25\point \PiSemGen[{\Bluecol #1[#2]}] n \else \PiSemGen[{\Bluecol #1[#2]}] n \fi}

 \def \PiLmuSem[#1]{\semPi{\LTerm<#1>}}

 \def \SPiLmuTerm[#1] #2 {\setbox200=\hbox{$#2$}%
\ifdim\wd200>1pt{\PiLmuSem[{#1}] \hskp {\picolour #2}}\else{\PiLmuSem[{#1}]\kern-.5\point}\fi}
 \def \BPiLmuSem[#1] #2 {\Bang {\semPi{\LTerm<#1>}<f>} {#2} }

 \def \BPiLmuLSem{\Bang \SPiLmuTerm}
 \def \BSPiLmuLTerm{\Bang \SPiLmuTerm}
 \def \BPiLmuTerm{\Bang \PiLmuTerm}
 \def \BSPiLmuTerm{\Bang \SPiLmuTerm}

 \def \PiLmuTerm [#1] #2 {\if@om \omfalse \PiLmuTermAux[#1] #2 \omtrue \resetvariables \else \PiLmuTermAux[#1] #2 \fi}

 \def \PiLmuTermAux[%]
 	{\@ifnextchar l{\PiLmuTermAbs[}%]
	{\@ifnextchar X{\PiLmuTermXpp[}%]
	{\@ifnextchar Y{\PiLmuTermYpp[}%]
	{\@ifnextchar a{\PiLmuTermapp[}%]
	{\@ifnextchar b{\PiLmuTermbpp[}%]
	{\@ifnextchar D{\PiLmuTermDlApp[}%]
	{\@ifnextchar d{\PiLmuTermdlApp[}%]
	{\@ifnextchar v{\PiLmuTermVar[}%]
	{\@ifnextchar ({\PiLmuTermBr[}%])
	{\@ifnextchar S{\PiLmuTermSub[}%]
	{\@ifnextchar s{\PiLmuTermsub[}%]
	{\@ifnextchar t{\PiLmuTermTub[}%]
	{\@ifnextchar c{\PiLmuTermContsub[}%]
	{\@ifnextchar C{\PiLmuTermContSub[}%]
	{\@ifnextchar F{\PiLmuTermContFSub[}%]
	{\@ifnextchar n{\PiLmuTermName[}%]
	{\@ifnextchar m{\PiLmuTermMu[}%]
	{\@ifnextchar U{\PiLmuTermMU[}%]
	{\@ifnextchar B{\PiLmuTermBot[}%]
		{%{\HL ?} 
		\SPiLmuTerm[}%]
}}}}}}}}}}}}}}}}}}}

 \def \PiExsub #1 := #2 {\setbox201=\hbox{\neww}%
	\New \copy201 ( \Out #1 <\copy201> . \PiLmuTerm [#2] \copy201 ) }
 \def \PiExSub #1 := #2 {\semPi {{#1}\skp{:=}\skp\LTerm<#2> } {} }

 \def \PiExContFSub #1 := #2 . #3 {\In #1 (v,d) . ( \Bang \PiExSub v := {#2} \Par \BEq d=#3 ) }
 \def \PiExContFsub #1 := #2 . #3 {\In #1 (v,d) . ( \Bang \PiExsub v := {#2} \Par \BEq d=#3 ) }
 \def \PiExContsub #1 := #2 . #3 {\In #1 (v,d) . ( \PiExSub v := {#2} \Par \BEq d=#3 ) }
 \def \PiExContSub #1 := #2 . #3 {\SPiLmuTerm [{}#1 := #2{`.}#3] {} }

% \def \PiLmuTermXpp[X #1 #2] #3 {\global\setbox103=\hbox{\newc}%
%\New \copy103 ( \PiLmuTermAux [#1] {\copy103} \Par \SPiLmuTerm [\copy103 := #2{`.}#3] {} ) }

 \def \PiLmuTermXpp[X #1 #2] #3 {\global\setbox103=\hbox{\newc}%
\New \copy103 ( \PiLmuTermAux [#1] {\copy103} \Par \Bang \PiExContFSub \copy103 := {#2} . {#3}] {} ) }

 \def \PiLmuTermYpp[Y #1 #2] #3 {\global\setbox103=\hbox{\newc}%
\New \copy103 ( \PiLmuTermAux [#1] {\copy103} \Par \Bang \setcounter{indw}{-1} \PiExContFsub \copy103 := {#2} . {#3}] {} ) }


 \def \PiLmuTermapp[a #1 #2] #3 {\global\setbox103=\hbox{\newc}%
\New \copy103 ( \PiLmuTermAux [#1] {\copy103} \Par \Bang 
% \Bang needed because of reduction of (`m`a.C)N 
\In {\copy103} (v{,}d) . ( \PiExSub v := {#2} \Par \BEq d={#3} ) ) }

 \def \PiLmuTermbpp[b #1 #2] #3 {\global\setbox103=\hbox{\newc}%
\New \copy103 ( \PiLmuTermAux [#1] {\copy103} \Par 
% \Bang \In {\copy103} (v{,}d) . ( \Bang \PiExsub v := {#2} \Par \BEq d={#3} ) 
\PiExContSub {\copy103} := {#2} . {#3}
) }

 \def \PiLmuTermDlApp[D #1 #2] #3 {\global\setbox104=\hbox{\newc}%
\New \copy104 ( \PiLmuTermAux [#1] {\copy104} \Par 
	{} \quad \\ \quad \hfill 
\Bang \In {\copy104} (v,d) . ( \PiExSub v := {#2} \Par \BEq d={#3} ) ) }

 \def \PiLmuTermdlApp[d #1 #2] #3 {\global\setbox105=\hbox{\newc}%
\New \copy105 ( \PiLmuTermAux [#1] {\copy105} \Par 
	{} \quad \\ \quad \hfill 
\Bang \In {\copy105} (v,d) . ( \Bang \PiExsub v := {#2} \Par \BEq d={#3} ) ) }

 \def \PiLmuTermAbs[l #1 . #2] #3 {%
 \picolour \global\setbox111=\hbox{\newb}%
\NewA #1\copy111 ( \PiLmuTermAux [#2] \copy111 \Par \Out{#3} <#1,\copy111> ) }

 \def \PiLmuTermAbs[l #1 . #2] #3 {%\theindb \theindc % LAbs
\global\Adv{\depth}{1} % \the\depth
\ifnum\depth=0\global\sbox{\An}{\hbox{$\picolour #3$}}\fi
\ifnum\depth=1\global\sbox{\Ai}{\hbox{$\picolour #3$}}\fi
\ifnum\depth=2\global\sbox{\Aii}{\hbox{$\picolour #3$}}\fi
\ifnum\depth=3\global\sbox{\Aiii}{\hbox{$\picolour #3$}}\fi
\ifnum\depth=4\global\sbox{\Aiv}{\hbox{$\picolour #3$}}\fi
\ifnum\depth=5\global\sbox{\Av}{\hbox{$\picolour #3$}}\fi
\ifnum\depth=6\global\sbox{\Avi}{\hbox{$\picolour #3$}}\fi
\ifnum\depth=7\global\sbox{\Avii}{\hbox{$\picolour #3$}}\fi
%
% \the\depth \theindb
% \stepcounter{indb}
\global\setbox174=\hbox{\newb} 
\NewA {{#1}}{\copy174} ( \PiLmuTermAux [#2] {\copy174} \Par
%.\usebox{\An}.\usebox{\Aii}.\usebox{\Aiii}.\usebox{\Aiv}.\usebox{\Av}.
%\usebox{\Avi}.\usebox{\Avii}.\usebox{\Aviii}.
\ifnum\depth<-1{A} \else \ifnum\depth<0{B} \else \ifnum\depth<1{C}\fi\fi\fi
\ifnum\depth=0{\Out \usebox{\Ai} <{#1},{\copy174}> }\fi
\ifnum\depth=1{\Out \usebox{\Ai} <{#1},{\box174}> }\fi
\ifnum\depth=2{\Out \usebox{\Aii} <{#1},{\copy174}> }\fi
\ifnum\depth=3{\Out \usebox{\Aiii} <{#1},{\copy174}> }\fi
\ifnum\depth=4{\Out \usebox{\Aiv} <{#1},{\copy174}> }\fi
\ifnum\depth=5{\Out \usebox{\Av} <{#1},{\copy174}> }\fi
\ifnum\depth=6{\Out \usebox{\Avi} <{#1},{\copy174}> }\fi
\ifnum\depth=7{\Out \usebox{\Avii} <{#1},{\copy174}> }\fi
\ifnum\depth=8{\Out \usebox{\Avii} <{#1},{\copy174}> }\fi
\ifnum\depth>8\Out #3 <{#1},b_{\the\depth}>\fi
) \global\Adv{\depth}{-1} \addtocounter{indb}{-1} % RAbs
}

 \def \PiLmuTermVar[v #1] #2 {\In {#1} (u) . \BEq u=#2 } %\In z (u) . \Out{#2} <u> 

 \def \PiLmuTermName[n #1 #2] #3 { \PiLmuTerm [#2] {#1} }

\def \Sink{\bullet}

% \def \PiLmuTermWSub[#1][#2/#3] #4 {\PiLmuTermAux [#1] #4 [#2/#3]  } 
 \def \PiLmuTermWSub[#1][#2/#3] #4 {\PiLmuTermAux [#1 {[#2/#3]}] #4   } 
 
% \textrm{\bf s}
% \def \PiLmuTermMu[m #1 . #2] #3 { \New \Sink#1 ( \PiLmuTerm[#2] {\Sink} \Par \BEq #1=#3 ) }
 \def \PiLmuTermMu[m #1 . #2] #3 { \New {\Sink} ( \PiLmuTermWSub[#2][#3/#1] {\Sink} ) }
 \def \PiLmuTermMU[U #1 . #2] #3 { \New {\Sink} ( \PiLmuTermAux[#2] {\Sink} ) }


 \def \PiLmuTermContsub[c #1 #2 := #3 . #4] #5 {\NewA #2 ( \PiLmuTermAux [#1] {#5} \Par {\Bang \PiExContsub #2 := {#3} . #4 } ) }
 \def \PiLmuTermContSub[C #1 #2 := #3 . #4] #5 {\NewA #2 ( \PiLmuTermAux [#1] {#5} \Par {\PiExContSub #2 := {#3} . #4 } ) }
 \def \PiLmuTermContFSub[F #1 #2 := #3 . #4] #5 {\NewA #2 ( \PiLmuTermAux [#1] {#5} \Par {\Bang \PiExContFsub #2 := {#3} . #4 } ) }

 \def \PiLmuTermSub[S #1 #2 := #3] #4 {\NewA #2 ( \PiLmuTermAux [#1] {#4} \Par \PiExSub #2 := {#3} ) }
 \def \PiLmuTermsub[s #1 #2 := #3] #4 {\NewA #2 ( \PiLmuTermAux [#1] {#4} \Par \Bang \PiExsub #2 := {#3} ) }
 \def \PiLmuTermTub[t #1 #2 := #3] #4 {\NewA #2 ( \PiLmuTermAux [#1] {#4} \Par 
 	{} \\ \quad \hfill
 \ExPiSub #2 := {#3} ) }

\def \PiLmuTermBot[B] #1 {\Zero}

\def \PiLmuTermBr[(#1)] #2 {\PiLmuTermAux [#1] #2 }


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Lmu full encoding
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def \LmuSyncell #1 [#2] #3 { \picolour \In {#2} (\Map v-d ) . ({ \BEq{#1}=v \Par \BEq d={#3} }) }
\def \LmuSynCell #1 [#2] #3 { \picolour \Bang \In {#2} (\Map v-d ) . ({ \BEq{#1}=v \Par \BEq d={#3} }) }

 \def \PiLmuFSem[#1]{\semPi{\LTerm<{#1}>}<f>}

 \def \SPiLmuFTerm[#1] #2 {\setbox200=\hbox{$#2$}%
\ifdim\wd200>1pt{\PiLmuFSem[{#1}] \hskp {\picolour #2}}\else{\PiLmuFSem[{#1}]\kern-.5\point}\fi}
 \def \BPiLmuFSem[#1] #2 {\Bang {\semPi{\LTerm<#1>}<f>} {#2} }

 \def \BPiLmuLSem{\Bang \SPiLmuTerm}
 \def \BSPiLmuLTerm{\Bang \SPiLmuTerm}
 \def \BPiLmuTerm{\Bang \PiLmuFTerm}
 \def \BSPiLmuTerm{\Bang \SPiLmuTerm}
 \def \BPiLmuFTerm{\Bang \PiLmuFTerm}

 \def \PiLmuFTerm [#1] #2 {\if@om \omfalse \PiLmuFTermAux[#1] #2 \omtrue \resetvariables \else \PiLmuFTermAux[#1] #2 \fi}

 \def \PiLmuFTermAux[%]
 	{\@ifnextchar l{\PiLmuFTermAbs[}%]
	{\@ifnextchar A{\PiLmuFTermApp[}%]
	{\@ifnextchar a{\PiLmuFTermapp[}%]
	{\@ifnextchar d{\PiLmuFTermDlApp[}%]
	{\@ifnextchar v{\PiLmuFTermVar[}%]
	{\@ifnextchar ({\PiLmuFTermBr[}%])
	{\@ifnextchar S{\PiLmuFTermSub[}%]
	{\@ifnextchar s{\PiLmuFTermsub[}%]
	{\@ifnextchar t{\PiLmuFTermTub[}%]
	{\@ifnextchar c{\PiLmuFTermContsub[}%]
	{\@ifnextchar C{\PiLmuFTermContSub[}%]
	{\@ifnextchar Z{\PiLmuFTermDlSub[}%]
	{\@ifnextchar n{\PiLmuFTermName[}%]
	{\@ifnextchar m{\PiLmuFTermMu[}%]
	{\PiLmuFSem[}%]
}}}}}}}}}}}}}}

 \def \ExFsub #1 := #2 {\PiLmuFTerm [#2] #1 }
 \def \ExFSub #1 := #2 {\BPiLmuFTerm [#2] #1 }
 \def \ExFContsub #1 := #2 . #3 {
\stepcounter{indb}\stepcounter{indc}
\New {\bind} ( \LmuSynCell {\bind} [#1] {#3} \Par \Bang \SPiLmuFTerm [#2] {\bind} )
\addtocounter{indb}{-1}\addtocounter{indc}{-1}
}
% \In #1 (v,d) . ( \BPiLmuFTerm [#2] v  \Par \BEq d=#3 ) }
 \def \ExFContSub #1 := #2 . #3 {\SPiLmuFTerm [{#1 := #2{`.}#3}] {} }

 \def \PiLmuFTermApp[A #1 #2] #3 {%\theindb \theindc % LApp
\setbox154=\hbox{$#3$}
\stepcounter{indb}\stepcounter{indc}
\New {\cind\bind} ( \PiLmuFTermAux [#1] {\cind} \Par \LmuSynCell {\bind} [{\cind}] {\box154} \Par \Bang \SPiLmuFTerm [#2] {\bind} )
\addtocounter{indb}{-1}\addtocounter{indc}{-1} % RApp
}

 \def \PiLmuFTermapp[a #1 #2] #3 {%\theindb \theindc % LApp
\setbox154=\hbox{$#3$}
\stepcounter{indb}\stepcounter{indc}
\New {\cind}{\bind} ( \PiLmuFTermAux [#1] {\cind} \Par 
% \Bang needed because of reduction of (`m`a.C)N 
\LmuSynCell {\bind} [{\cind}] {\box154} \Par \Bang \SPiLmuFTerm [#2] {\bind} )
\addtocounter{indb}{-1}\addtocounter{indc}{-1} % RApp
}

 \def \PiLmuFTermDlApp[d #1 #2] #3 {%\theindb \theindc % LApp
\setbox154=\hbox{$#3$}
\stepcounter{indb}\stepcounter{indc}
\New {\cind}{\bind} ( \PiLmuFTermAux [#1] {\cind} \Par 
	\quad {} \\ \hfill
\LmuSynCell {\bind} [{\cind}] {\box154} \Par \Bang \SPiLmuFTerm [#2] {\bind} )
\addtocounter{indb}{-1}\addtocounter{indc}{-1} % RApp
}

 \def \PiLmuFTermAbs[l #1 . #2] #3 {\picolour \setbox111=\hbox{\newb}%
\NewA #1\copy111 ( \PiLmuFTermAux[#2] \copy111 \Par \Out{#3} <#1,\copy111> ) }

 \def \PiLmuFTermVar[v #1] #2 {\BEq #1=#2 } % \In #1 (u) . \Out{#2} <u> 

 \def \PiLmuFTermName[n #1 #2] #3 { \PiLmuFTermAux[#2] {#1} }

 \def \PiLmuFTermMu[m #1 . #2] #3 { \New \Sink#1 ( \PiLmuFTermAux[#2] {\Sink} \Par \BEq #1=#3 ) }

 \def \PiLmuFTermContsub[c #1 #2 := #3 . #4] #5 {\NewA #2 ( \PiLmuFTermAux [#1] {#5} \Par {\Bang\ExFContsub #2 := #3 . #4 } ) }

 \def \PiLmuFTermContSub[C #1 #2 := #3 . #4] #5 {\NewA #2 ( \PiLmuFTermAux [#1] {#5} \Par {\ExContSub #2 := #3 . #4 } ) }

 \def \PiLmuFTermSub[S #1 #2 := #3] #4 {\NewA #2 ( \PiLmuFTermAux [#1] {#4} \Par \BPiLmuFTerm [#3] #2 ) }

 \def \PiLmuFTermsub[s #1 #2 := #3] #4 {\NewA #2 ( \PiLmuFTermAux [#1] {#4} \Par \Bang \ExFsub #2 := {#3} ) }

 \def \PiLmuFTermTub[t #1 #2 := #3] #4 {\NewA #2 ( \PiLmuFTermAux [#1] {#4} \Par 
 	{} \\ \quad \hfill
 \exsub #2 := #3 ) ) }

 \def \PiLmuFTermDlSub[Z #1 #2 := #3] #4 {\NewA #2 ( \PiLmuFTermAux [#1] {#4} \Par \\ \hfill \Bang \SPiLmuTerm [{#3}] #2 ) }

\def \PiLmuFTermBr[(#1)] #2 {\PiLmuFTermAux [#1] #2 }


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\def \sequivalence{\mathrel{\stackrel{\bullet}{\sim}}}
\def \sbisimilaritytwo{\mathrel{\sim_{`p}}}

%

\def \Input{\textsl{input}}
\def \Output{\textsl{output}}

\def \CL{\textsc{cl}}

\makeatother

%])}

